Granular Synchrony

Today's mainstream network timing models for distributed computing are synchrony, partial synchrony, and asynchrony. These models are coarse-grained and often make either too strong or too weak assumptions about the network. This paper introduces a new timing model called granular synchrony that models the network as a mixture of synchronous, partially synchronous, and asynchronous communication links. The new model is not only theoretically interesting but also more representative of real-world networks. It also serves as a unifying framework where current mainstream models are its special cases. We present necessary and sufficient conditions for solving crash and Byzantine fault-tolerant consensus in granular synchrony. Interestingly, consensus among $n$ parties can be achieved against $f \geq n/2$ crash faults or $f \geq n/3$ Byzantine faults without resorting to full synchrony.

==> bft-async-proof.tex <==
\section{BFT Fine-grained Synchrony with Asynchrony}

\begin{theorem}
If BFT consensus on graph family $G_f$ is solvable, then for every graph $G\in G_f$ and any set $F$, where $|F|\leq f$, removing all asynchronous edges, $F$, and the largest connected component in graph $G-F$ must leave $k<n-|F|-f$ nodes in the remaining graph.
\end{theorem}

\begin{proof}
Suppose for the sake of contradiction there exists an algorithm $A$ which solves BFT consensus for $G_f$, such that there exists a graph $G\in G_f$ and a set $F$ ($|F|\leq f$), such that removing all asynchronous edges, all nodes in $F$, and the largest remaining connected component in $G$ leaves $k \geq n-|F|-f$ remaining nodes.

We define the following sets: $C_i$ is the set of nodes corresponding to the $i$-th connected component of $G-F$, where asynchronous edges are removed. We also define the set $F_i\subseteq F$, where $|F_i|=|F|-|C_i|$. In other words, $F_i$ is a subset of $F$, such that $|C_i\cup F_i|=|F|$.

We construct $q$ worlds ($w_1$, $w_2$, ..., $w_q$). In world $w_i$, we define the following graph $G_i$. $G_i$ is a vertex permutation of graph $G$, where $C_i$ and $F$ are swapped. If $|C_i|>|F|$, then $|C_i|-|F|$ nodes remain in $C_i$ (are not swapped). If $|F|>|C_i|$, then $|F|-|C_i|$ nodes remain in $F$ (are not swapped).

We define this vertex permutation as $\pi_i$. Note that since $G\in G_f$, $G_i\in G_f$ because $G_i$ is a vertex permutation of $G$. In world $w_i$, the adversary corrupts $C_i \cup F_i$. Note that $|C_i\cup F_i|=|F|\leq f$. $C_i$ behaves identically to correct behavior of $C_i$ in world $w_f$ when sending messages to $F$. $C_i$ also behaves identically to correct behavior of $C_i$ in world $w_j$ when sending messages to $C_j$. $F_i$ behaves identically to how it behaved in world $w_f$ (including simulating synchrony to other nodes in $F$). At time $t$, $C_i$ acts crashed. We also define a world $w_f$, for which the adversary corrupts $F$. $F$ behaves correctly until time $t$. At time $t$, $F$ acts crashed. Since algorithm $A$ solves consensus for $G_f$ (including any vertex permutation of $G$), when up to $f$ nodes are Byzantine faulty, algorithm $A$ solves BFT consensus in each of these worlds.


We construct an external system consisting of $q$ nodes connected only by asynchronous links. External node $q_i$ simulates the behavior of $C_i$ in world $w_i$. External node $q_f$ simulates $F$ in world $w_f$. 

Now suppose the external adversary crashes node $q_j\neq q_f$ at time $t$. We argue this execution is indistinguishable from world $w_j$. From the perspective of all $C_k\neq C_i$, $C_i$'s behavior in world $j$ is indistinguishable from $C_i$'s behavior in world $i$. $q_j$'s behavior exactly matches the behavior of of $C_j$ in world $j$. Thus, this execution in the external world is indistinguishable from world $j$. Since consensus is satisfied in world $j$ it is also satisfied in this external world when the adversary crashes $q_j\neq q_f$.

If the adversary crashes node $q_f$ at time $t$, then we argue this execution is indistinguishable from world $w_f$. $C_i$'s behavior in world $w_i$ simulates the correct behavior of $C_i$ in world $w_f$, therefore from the perspective of all $C_k\neq C_i$, $C_i$'s behavior in world $w_i$ is indistinguishable from its behavior in world $w_f$. Since consensus is satisfied in world $w_f$, it is also satisfied when the external adversary crashes $q_f$.

In both cases consensus is solvable in the external system when the adversary can crash up to one node, contradicting the FLP result.


%In world $w_i$, $C_i$ behaves identically as $C_i$ in world $w_j$ when sending messages to $C_j$. Thus, from $C_j$'s perspective $C_j$ cannot distinguish $C_i$'s behavior in world $w_j$ from world $w_i$. Furthermore, the behavior of $C_i$ when sending messages to $C_k$ in world $i$ is indistinguishable from the behavior of $C_i$ when sending messages to $C_k$ in world $j$. Thus, from $C_k$'s perspective $C_k$ cannot distinguish $C_i$'s behavior in world $w_j$ from world $w_i$.



%We define a sequence of worlds each with a different permutation of node labels for graph $G$. World hybrid has some initial labelling of the graph. Let $H=\pi(G)$, where $\pi$ is the labelling function. Now we define world $i$ to have the following labelling $\pi_i$. The first $|F|$ nodes in the $i$-th connected component of $H-\pi(F)$ are swapped with $\pi(F)$, while the other nodes remain the same.

%Now consider an external world, for which every node is connected by asynchronous links. Node $N_j$ in the external world simulates the nodes in the $j$-th connected component of graph $H-\pi(F)$ (graph $H$ without $\pi(F)$). Finally, the last external node, $N_f$ simulates nodes in $\pi(F)$. We now argue that algorithm $A$ solves CFT consensus in this external world, where up to one of the nodes can crash, contradicting the FLP result. There are two cases: 1) the adversary in the external world crashes $N_f$ at time $t$ and 2) the adversary in the external world crashes node $N_j\neq N_f$ at time $t$. 


%For case 1, world hybrid has, $H$, the labelled graph that corresponds to the simulation by the external nodes. Algorithm A must solve consensus for any set of up to $f$ corrupted nodes, in any labelling of $G$. Therefore, algorithm A must solve consensus in world hybrid if the adversary crashes $\pi(F)$ at time $t$. This corresponds to crashing $N_f$ in the external world, so nodes in the external world will also reach consensus if the adversary crashes $N_f$ at time $t$. 


%For case 2, let $S_j$ be the set of nodes $N_j$ simulates (the $j$-th connected component of $H-\pi(F)$). World $j$ has a labelled graph such that $\pi_j(F)\subseteq S_j$ and $S_j-\pi_j(F)$ are in the same connected component. The adversary in world $j$ crashes $S_j-\pi_j(F)$ (if non-empty) at time $0$ and corrupts $\pi_j(F)$ at time $t$. Note this is a corruption of $|S_j|$ nodes, which is at most $f$ (any connected component must be of size at most $f$ by theorem assumption). The adversary in world $j$ controls all nodes in $\pi_j(F)$, and the message delay, so it respects any synchrony assumptions between $\pi_j(F)$ and other correct nodes in world $j$. This corresponds to the adversary in the external world crashing $N_j$ at time $t$. 
\end{proof}

Example with connected components bigger than |F|:
Here is a similar example where n=11, f=4, and |F|=3 (|F|<f). and the other connected components are of size 4.

Graph H1: 456A - 123 - 789B
Define the following sets: F1={123}, CC1={456A}, CC2={789B}

Graph H2: 123A - 456 - 789B
Define the following sets: F2={456A}, CC1={123}, CC2={789B}

Graph H3: 123B - 789 - 456A
Define the following sets: F3={789B}, CC1={123}, CC2={456A}

In graph H1, F1 (nodes 123) is Byzantine faulty. Consider this execution (E1). F1 simulates the correct behavior of CC1 in graph H2 when communicating with nodes 456A. And it simulates the correct behavior of CC1 in graph H3 when communicating with nodes 789B.

In graph H2, F2 (nodes 456A) is Byzantine faulty. Consider this execution (E2). F2 simulates the correct behavior of CC1 in graph H1 when communicating with nodes 123. And it simulates the correct behavior of CC2 in graph H3 when communicating with nodes 789B.

In graph H3, F3 (nodes 789B) is Byzantine faulty. Consider this execution (E3). F3 simulates the correct behavior of CC2 in graph H1 when communicating with nodes 123. And it simulates the correct behavior of CC2 in graph H2 when communicating with nodes 456.

Now we will construct three external nodes: Q1, Q2, and Q3. Q1 will simulate F1 (nodes 123) in graph H1 under execution E1. Q2 will simulate F2 (nodes 456A) in graph H2 under execution E2. Q3 will simulate F3 (nodes 789B) in graph H3 under execution E3. I argue this is a faithful simulation. From Q1's perspective, Q2 and Q3 are behaving exactly like correct nodes would do in H1. Similarly from Q2's perspective, Q1 and Q3 behave exactly like the correct nodes do in H2. And from Q3's perspective, Q1 and Q2 behave exactly like correct nodes do in H3.


==> bft-gps-analysis.tex <==
\section{Analysis of BFT consensus protocol in \gpscaps}\label{bft-gps-analysis}
External validity is easily ensured if all correct nodes validate the proposed value before voting for it. We focus on agreement and termination. 

\begin{lemma}\label{lem:hps-bft-agree-1}
If there exist $n-f$ \msg{Vote-1}{v,val} messages and $n-f$ \msg{Vote-1}{v,val'} messages in the same view $v$, then $val=val'$.
\end{lemma}

\begin{proof}
Suppose for the sake of contradiction there exist a set $S$ of $n-f$ \msg{Vote-1}{v,val} messages and a set $S'$ of $n-f$ \msg{Vote-1}{v,val'} messages where $val\neq val'$. 

Of the $n-f$ nodes whose \textsc{Vote-1} messages are in $S$, at least a set $P$ of $n-2f$ must be correct. 
By the condition in theorem~\ref{thm:bft-gps}, $P \rightarrow H$ where $H$ is a set of $f+1$ correct nodes. 
Due to quorum intersection, $S'\cap H$ must contain at least one node, which is correct. 
Let $c'$ be this node.
Since the graph is undirected, there exists $c \in S$ such that $c' \rightarrow c$. 

Let $t$ be the time $c'$ starts its vote timer. 
At time $t$, $c'$ also forwards the \msg{Propose}{v,val',-} message to all nodes. 
By time $t+d\Delta$, $c$ receives this message.
Thus, $c$ must have sent \msg{Vote-1}{v,val} before time $t+d\Delta$.
Otherwise, $c$ would have detected leader equivocation and would not have voted. 
Then, $c$ must have forwarded \msg{Propose}{v,val,-} to all nodes before time $t$.
$c'$ receives this \msg{Propose}{v,val,-} message before time $t+d\Delta$, which is before its vote timer expires. 
Thus, $c'$ detects leader equivocation and would not have voted. 
This contradicts $c' \in S'$. 
\end{proof}

%\begin{lemma}\label{lem:hps-bft-agree-2}
%If a correct node commits $val$ in view $v$, then at least $f+1$ correct nodes update their $lock \gets (v,val,-)$ before entering a view higher than $v$.
%\end{lemma}

%\begin{proof}
%If a correct node commits $val$ in view $v$, it must have received $n-f$ \msg{Vote-2}{v,val} messages.
%Of the $n-f$ nodes who sent \msg{Vote-2}{v,val}, at least a set $P$ of $n-2f$ must be correct.
%Due to the condition in the theorem, $P \rightarrow Q$ where $Q$ is a set of $f+1$ correct nodes. 
%We now show that every node $q\in Q$ sets its $lock=(v,val,-)$ before entering a higher view.

%Since the graph is undirected, there exists $p \in P$ such that $q \rightarrow p$. 
%Let $t_q$ be the time node $q$ receives a blame certificate for view $v$ or higher. Node $q$ forwards the blame certificate to all nodes at time $t_q$, which reaches node $p$ by time $t_q+d\Delta$. 
%Thus, $p$ must have sent its \msg{Vote-2}{v,val} message before time $t_q+d\Delta$, at which time it also sets and sends its $lock=(v,val,-)$.
%Node $q$ will receive $p$'s lock by time $t_q+2d\Delta$, which is still within its waiting period before entering view $v+1$ or higher.
%Thus, node $q$ will update its $lock=(v,val,-)$ before entering a view higher than $v$.
%\end{proof}

\begin{lemma}\label{lem:hps-bft-agree-2}
If some node commits $val$ in view $v$, then any set of $n-f$ \msg{Vote-1}{v',val'} messages (lock certificate) in view $v'\geq v$ must have $val'=val$.
\end{lemma}

\begin{proof}
We prove this lemma by induction on view $v'$. 
The base case of $v'=v$ is straightforward by lemma \ref{lem:hps-bft-agree-1}. 
For the inductive step, suppose the lemma holds up to view $v'-1$, and now we consider view $v'$. Suppose for the sake of contradiction that some node commits $val$ in view $v$, and there exist $n-f>f$ nodes that send \msg{Vote-1}{v',val'} messages for $val' \neq val$.
%This means that at least a set of $n-f$ nodes received a \msg{Propose}{v',val',S} message and sent a \msg{Vote-1}{v',val'} message, of which at least $n-2f\geq 1$ must be correct (since $n\geq 2f+1$, $n-2f\geq 1$). %Since $L_{v'}$ sends \msg{Propose}{v',val'}, there must exist a set $P$ of $n-f$ nodes that have received $f+1$ \msg{ViewChange}{v'} messages and waited $2d\Delta$ before entering view $v'$. 
A correct node will only send \msg{Vote-1}{v',val'} if a proposal carries in view $v'$ a set $S$ of \msg{Status}{v',-} messages. 
Thus, there exists a subset $H\subseteq S$ of $n-2f$ correct nodes which sent \msg{Status}{v',-}. 
By the condition in theorem~\ref{thm:bft-gps}, $H\rightarrow Q$, where $Q$ is a set of $f+1$ correct nodes. 


%\neil{punch line is that n-2f correct status hears from f+1 correct, then f+1 correct must intersect n-2f locked}


Since a node committed $val$ in view $v$, there must exist some set $n-f$ nodes that sent \msg{Vote-2}{v, val}, of which a set $R$ of at least $n-2f$ are correct. 
Before sending \msg{Vote-2}{v,val} messages, these correct nodes updated $lock\coloneqq (v,val)$ in view $v$. Sets $Q$ and $R$ intersect in at least one correct node. Let this node be $q$. Since the graph is undirected and $H\rightarrow Q$, there must exist a node $h\in H$ such that $q\rightarrow h$. By the induction hypothesis, any lock certificate from view $v$ to $v'-1$ must be for $val$. Since a node only updates its lock monotonically based on view numbers, node $q$ must have a lock with view $\geq v$ for $val$. 
Let $t_h$ be the time node $h$ echoed $f+1$ \msg{ViewChange}{v'} messages. By time $t_h+d\Delta$, node $q$ must have received $f+1$ \msg{ViewChange}{v'} messages. Node $q$ will then echo a \msg{Locked}{lock} message to all nodes. This will be received by node $h$ by time $t_h+2d\Delta$. Node $h$ will update its lock to be at least view $v$ for $val$. 
Thus, from nodes in $H$, $L_{v'}$  receives at least one \textsc{Status} message for $val$ with view $\geq v$. By the induction assumption, any lock certificate not for $val$ must have view $<v$. 
Thus, no correct node sends \msg{Vote-1}{v',val'}, a contradiction.
%Since a lock certificate formed for $val'$ in view $v'$, at least one correct node must have sent a \msg{Vote-1}{v',val'}, a contradiction because a correct node will only vote for $val$ in view $v'$.
\end{proof}

%\begin{lemma}
%If a node commits $val$ in view $v$, then any set of $n-f$ \msg{Vote-1}{v',val'} messages (lock certificate) in view $v' \geq v$ must have $val'=val$.
%\end{lemma}

%\begin{proof}
%We prove this lemma by induction. The base case is established by lemma~\ref{lem:hps-bft-agree-1}.
%For the inductive step, suppose the lemma holds up to view $v'-1$, and now we consider view $v'$.
%By lemma \ref{lem:hps-bft-agree-2}, there are at least $f+1$ correct nodes who have set $lock=(v,val,-)$. 
%By the induction hypothesis, any lock certificate for any view between $v$ and $v'-1$ must be for $val$. 
%By quorum intersection, the set of $n-f$ \msg{Status}{v',-} messages in the leader's proposal in view $v'$ must contain at least one lock for $val$ from view $v$ or higher.
%Thus, correct nodes will only vote for $val$ in view $v'$.
%Thus, any set of $n-f$ \msg{Vote-1}{v',val'} messages (lock certificate) must have $val'=val$.
%\end{proof}

\begin{theorem}[Agreement]
No two correct nodes commit different values.    
\end{theorem}

\begin{proof}
Let $v$ be the smallest view in which a correct node commits some value, say $val$. 
By lemma~\ref{lem:hps-bft-agree-2}, only $val$ can receive $n-f$ \msg{Vote-1}{v} messages in any view $v' \geq v$, so no other value can be committed by a correct node.
\end{proof}

%\begin{lemma}
%A correct node eventually reaches a view $v$, where $L_v$ is correct, after $GST+2d\Delta$.    
%\end{lemma}

% TODO change to an induction argument
%\begin{proof}
%Let $v'$ be the largest view of any correct node at time $GST$. To enter view $v'$ this correct node must have received a blame certificate for view $v'-1$. This correct node forwarded this blame certificate to all nodes at some time $\leq GST$ to all nodes. All correct nodes will receive this blame certificate by time $GST+\Delta$ and enter view $v'$ by time $GST+(2d+1)\Delta$. Eventually, at least $f+1$ correct nodes will timeout view $v'$ and send a \msg{Blame}{v'} message to all nodes. Eventually, a correct node will receive $f+1$ \msg{Blame}{v'} messages and enter view $v'+1$ $2d\Delta$ time afterwards. If the leader of view $v'+1$ is correct, then the lemma is satisfied. Otherwise, by a similar argument correct nodes will keep entering increasing views until it reaches view $v$.
%\end{proof}

\begin{theorem}[Termination]
All correct nodes eventually decide.    
\end{theorem}

\begin{proof}
With round-robin leader election, correct nodes are elected leaders infinitely often. Thus, there must be a view $v$, after $GST+2d\Delta$, whose leader is correct. We next prove that all nodes will decide and terminate in view $v$ (if they don't decide earlier). 


Let $t$ ($t \geq GST+2d\Delta$) be the first time some correct node enters view $v$. 
This correct node echoes $f+1$ \msg{ViewChange}{v-1} messages to all nodes at $t-2d\Delta \geq GST$. 
All correct nodes will receive the new view certificate by time $t-2d\Delta+\Delta$, wait $2d\Delta$ themselves, and enter view $v$ by time $t+\Delta$. 
Upon entering view $v$, they send \msg{Status}{v,-} messages to $L_v$. 
$L_v$ receives $n-f$ \msg{Status}{v,-} messages by time $t+2\Delta$, and send a \msg{Propose}{v,-} message to all nodes. 
All correct nodes will receive the \msg{Propose}{v,-} message by time $t+3\Delta$ and start their vote timers. 
Since $L_v$ is correct and does not equivocate, all correct nodes will send a \msg{Vote-1}{v,-} message by time $t+(3+d)\Delta$. 
All correct nodes will receive $n-f$ \msg{Vote-1}{v,-} messages by time $t+(4+d)\Delta$, and send a \msg{Vote-2}{v,-} message.
All correct nodes will receive $n-f$ \msg{Vote-2}{v,-} messages and commit by time $t+(5+d)\Delta)$. 
Since a node's view timer is $(5+d)\Delta$, and changing views requires $f+1$ \msg{ViewChange}{v} messages, all correct nodes will remain in view $v$, commit and terminate in view~$v$.
\end{proof}

%\rl{decide if we go for external validity of unanimity}\neil{i vote for keeping external validity and putting unanimity in the appendix}

%\rl{next section can be short, I think. The modification and proof are almost the same as in the CFT case.}

==> disc_2024/async-psync-sync-bft-proofs.tex <==
\section{HAPS BFT Consensus Proofs}

\subsection{Agreement}

\subsection{Termination}
The adversary must let at least one correct $\diamond f+1$-correct-bisource always exist in the underlying communication graph. If there are multiple correct $\diamond f+1$-correct-bisources then let $L_v$ be a correct bisource which remains a correct bisource throughout the execution of the protocol.

\begin{lemma}
Let view $v$ be the first view after GST for which $L_v$ is elected leader. If no correct node terminates in view $v'<v$, then all correct nodes will reach view $v$.
\end{lemma}

\begin{proof}
We prove the lemma by induction on view $v$.

\par \textbf{Base Case:} $v=1$. All correct nodes start in view $1$, so they reach view $1$ trivially.

\par \textbf{Induction Step.} By the induction assumption we assume no correct node terminates in an earlier view, and all correct nodes reach view $v-1$.

Suppose for the sake of contradiction no correct node terminates in view $v-1$, and at least one correct node never reaches view $v$. If a correct node never reaches view $v$ then it must have never received $n-f$ \msg{Blame}{v-1} messages. 

This implies that at least one correct node never sends a \msg{Blame}{v-1} message. This correct node, $n_1$, must have never received $n-f$ \msg{Blame}{v-1} messages, since $n_1$ would have forwarded the blame certificate to all correct nodes, and they would all eventually advance to view $v$. Instead node $n_1$ must have received a \msg{Propose}{v-1,-,-} message before its echo timer expired (otherwise it would have sent a \msg{Blame}{v-1} message, a contradiction). It then would have echoed the \msg{Propose}{v-1,-,-} message to all nodes, and started its vote timer. It must have sent a \msg{Vote-1}{v-1,-} message to all nodes (otherwise it would have detected equivocation and sent a \msg{Blame}{v-1} message, a contradiction). 

\par We now show that all correct nodes must have sent a \msg{Vote-1}{v-1,-} message. Suppose not, then there must be at least one correct node, $n_2$, which did not send a \msg{Vote-1}{v-1,-} message. Node $n_2$ will eventually receive a \msg{Propose}{v-1,-,-} from node $n_1$. It then will start its vote timer. Since node $n_2$ never sends a \msg{Vote-1}{v-1,-} message, it must have detected equivocation before its vote timer expired. Node $n_2$ will then have forwarded the equivocation to all nodes, which means node $n_1$ must eventually receive the equivocation. Node $n_1$ will then send a \msg{Blame}{v-1} message, a contradiction to the assumption that $n_1$ never sends a \msg{Blame}{v-1} message.

\par Since all correct nodes must have sent a \msg{Vote-1}{v-1,-} message, all correct nodes will eventually receive $n-f$ \msg{Vote-1}{v-1,-} messages. All correct nodes will then send a \msg{Vote-2}{v-1,-} message to all nodes. Therefore, all correct nodes, including node $n_1$ will eventually receive $n-f$ \msg{Vote-2}{v-1,-} messages and commit, a contradiction to the assumption that no correct node terminates in view $v-1$.
\end{proof}

\begin{lemma}
If all correct nodes enter view $v$, then they all terminate in view $v$.
\end{lemma}

\begin{proof}
When all correct nodes enter view $v$, they send a \textsc{Status} message to all nodes. Thus, all correct nodes will eventually receive $n-f$ \textsc{Status} messages, compute the highest lock and send a \textsc{Forward-HighestRanked} message to all nodes. Any correct node will echo the \textsc{Forward-HighestRanked} message to all nodes (if it has not done so already). Let $B$ be the set of $f+1$ correct nodes which have partially synchronous fault-free paths to $L_v$. Since view $v$ is after GST, and every node in $B$ has a partially synchronous fault-free path to $L_v$, every node in $B$ will receive a \textsc{Propose} message from $L_v$ before their echo timer expires, and forward the \textsc{Propose} message to all nodes for an equivocation check. $L_v$ is correct so it will not equivocate, therefore no node in $B$ will send a \msg{Blame}{v} message. Since a blame certificate requires at least $n-f$ nodes to send a \textsc{Blame} message, and $f+1$ nodes in $B$ will not send a \msg{Blame}{v} message, no blame certificate will ever form in view $v$. Thus eventually all correct nodes will send a \textsc{Vote-1} message, and receive $n-f$ \textsc{Vote-1} messages. Therefore, all correct nodes will send a \textsc{Vote-2} message, and receive $n-f$ \textsc{Vote-2} messages, and terminate in view $v$.
\end{proof}

\begin{theorem}
HAPS BFT satisfies termination.
\end{theorem}

\begin{proof}
If at some point some correct node terminates, it will send a \textsc{Commit} message to all nodes. This message is sent by a correct node, so all correct nodes will eventually receive the message and terminate as well. Now assume that no correct node terminates in any view $v'<v$. In that case by lemma \ref{} all correct nodes eventually reach view $v$. Then by lemma \ref{} all correct nodes terminate during view $v$.
\end{proof}

\subsection{Validity}

%Easy way is to use an off the shelf CFT consensus protocol with n>2f and partially synchronous and then we are done
%the main downside is the replication factor
%if the adversary is a bit weaker can we do better

%The worst case is the adversary corrupts all links
%Unlikely in practice the adversary will corrupt all links to be psync
%We know from section 3 that all
%Necessary condition - Give examples of in practice: for example if n=f+1 then the adversary cannot corrupt any links, if n=2f+1 the adversary can corrupt all links
%HPS is more flexible framework, it aligns
%The next question is does it help, what can we do with it? what is true? is consensus still possible in hps. In sync/psync we understand when consensus is possible or not, our first step is to establish those results for this model
%we can instantiate replication factor bounds depending on the adversary
%give a table of different values

%section 4
%we know consensus is possible in HPS
%we need to design an algorithm that actually
%the obvious strategy, is to use a partially synchronous protocol because in the worst case it psync protocol
%other extreme the adversary corrupts 0 links we know of existing cft sync protocols
%the interesting space is in between the sync and psync extremes
%we're interested in what algorithm we can design for $n<=2f$, for $n>2f$ we can use psync
%add adversary can corrupt up to t paths/links, then in section 3 say
%if cft consensus is solvable then any t links the adversary corrupts such that for all V', V' V' is at least f+1 synchronous
%add a couple of examples to link it back to the t parameter,
%if n=f+1, then any node must have f+1 edges so t must be 0
%if n=2f+1, then f+1 nodes must need at least f+1 sync connections

%show figure examples for synchronous path/k-synchronous, and bisource

==> disc_2024/async-psync-sync-impossibility.tex <==
\section{Necessary Conditions for BFT Consensus}\label{s:bft-necessary}





\subsection{Necessary Condition for BFT Consensus under HAPS}\label{s:haps-bft-necessary}
Next we prove that theorem \ref{thm:haps-bft-necessary} is a necessary condition for solving BFT consensus under HAPS.
%\begin{lemma}
%There does not exist a BFT consensus algorithm for any graph which contains a subset $V'\subset V$ of correct nodes, where $|V'|=n-2f$, has synchronous fault-free paths in $G'=(V-F,E_{sync})$ to at most $f$ correct nodes.

%If there exists a BFT consensus algorithm uner the HAPS model tolerating at most $f$ Byzantine fault nodes and $s$ link alterations, then any subset $V'\subset V$ of correct nodes, where $|V'|=n-2f$, has synchronous fault-free paths in $G'=(V-F,E_{sync})$ to at least $f+1$ correct nodes.
%\end{lemma}

%\begin{proof}
%Suppose for the sake of contradiction there does exist a BFT consensus algorithm for any graph $G$, where in $G$ there exists a subset $V'\subset V$ of correct nodes, where $|V'|=n-2f$, has synchronous fault-free paths in $G'=(V-F,E_{sync})$ to at most $f$ correct nodes.

%\begin{itemize}
%    \item $S$ is the set of $f$ correct nodes $V'$ has paths to. $|S|=f$.
%    \item $T=V-S$ is the set of remaining correct nodes not in $S$. $|T|=n-2f$.
%    \item $F$ is the set of faulty nodes. $|F|=f$.
%\end{itemize}

%Note that $|S|+|T|=n-f$ and $|T|+|F| = n-f$. Since $n\leq 3f$, $|T|\leq f$.

%$S$, $T$, $F$ are all disjoint sets such that their union is the total number of vertices $V$.

%We now construct a hybrid argument and use indistinguishability to reach a contradiction.

%\textbf{World 1.} All nodes in $S\cup F$ are non-faulty and have input $x$. All nodes in $T$ are faulty and act crashed. By agreement, validity, and termination properties of the algorithm, all nodes in $S$ must decide $x$ by some finite time $T_1$.

%\textbf{World 2.} All nodes in $T\cup F$ are non-faulty have input $y$. All nodes in $S$ are faulty and act crashed. By agreement, validity, and termination properties of the algorithm, all nodes in $T$ must decide $y$ by some finite time $T_2$.

%\textbf{World Hybrid.} Nodes in $S$ have input $x$. Nodes in $T$ have input $y$. All nodes in $S$ and $T$ are non-faulty. All nodes in $F$ are Byzantine faulty. All messages sent between nodes in $S$ are delivered immediately. Nodes in $F$ act how they act in World 1 to $S$ (as if they have input $x$). Nodes in $F$ act how they act in World 2 to $T$ (as if they have input $y$). All messages sent between nodes in $T$ are delivered immediately. All messages sent between nodes in $S$ are delivered immediately. All messages sent from a node in $S$ to a node in $T$ or from a node in $T$ to a node in $S$ are delivered some time after $max(T_1, T_2)$. By the termination property $S$ must decide by time $T_1$. From the perspective of nodes in $S$, however, World 1 and World Hybrid are indistinguishable since nodes act the same in both worlds. So since $S$ decided $x$ in World 1, $S$ must decide $x$ in World Hybrid. Similarly, by the termination property $T$ must decide by time $T_2$. From the perspective of nodes in $T$, however, World 2 and World Hybrid are indistinguishable since nodes act the same in both worlds. Since $T$ decided $y$ in World 2, $T$ must decide $y$ in World Hybrid. This, violates the agreement property of the algorithm, a contradiction.
%\end{proof}

\begin{lemma}\label{lem:haps-helper-1}
If there exists a BFT consensus algorithm under the HAPS model tolerating at most $f$ Byzantine faults and $s$ link alterations, then there must exist a node which is correct and a $\diamond f+1$-correct-bisource in the underlying communication graph.
%There does not exist a BFT consensus algorithm for any graph which does not contain a correct $\diamond f+1$-correct-bisource.
\end{lemma}

\begin{proof}
Suppose for the sake of contradiction that there exists a BFT consensus algorithm for any graph that does not have a correct $\diamond f+1$-correct-bisource. By theorem \ref{thm:haps-bft-necessary}, any subset $V'\subset V$ with $|V'|=n-2f$ must be at least $f+1$-correct-synchronous.

We show how to solve consensus with one failure using this BFT consensus algorithm (contradicting FLP). Consider a set, $P$, of $\lceil n/f \rceil$ nodes, of which one node is faulty, and there are only asynchronous links between nodes. We construct a graph $G_1$, for which every node in $P$ has synchronous edges to $f-1$ correct dummy nodes. As every correct node is in $P$, and has synchronous edges to only nodes in $Q$ (containing $f-1$ nodes), there does not exist a correct $\diamond f+1$-bisource. 

%We now show that any subset $V'\subset V$ of correct nodes with $|V'|=n-2f$ has synchronous fault-free paths to at least $f+1$ correct nodes in $G_1$. There are two cases: 1) $n-f=1$ or 2) $n-f>1$. If $n-f=1$, then by lemma 2 $G$ must contain a correct $\diamond f+1$-bisource, a contradiction. Therefore, $n-f>1$. Any node in $Q$ has synchronous fault-free paths to all $n$ nodes, and any node in $P$ has synchronous fault-free paths to $f$ nodes. Therefore any set of $n-f$ nodes will have synchronous fault-free paths to at least $f+1$ nodes.

By assumption there must exist an algorithm, $A$, that solves BFT consensus for graph $G_1$. To solve consensus among nodes in $P$ with only asynchronous edges, nodes in $P$ just execute $A$ pretending that the graph is $G_1$, where $Q$ is just a set of dummy nodes that are crashed from the beginning. $A$ therefore solves consensus in an asynchronous network with one failure, a contradiction of the FLP result~\cite{flp}. 
\end{proof}

% no f+1 correct clique because that's a bisource, make every node an f psync bisource, f+1 - (n-2f) = f+1-n+2f = 3f+1-n,
%graph for which n-2f is connected to f+1 correct but no single node is connected to f+1 correct, except for n-2f=1
%n-2f+n-2f-(n-f) = 2n-4f-n+f = n-3f=intersection, so no intersection between n-2f

%\begin{theorem}
%Suppose there exists a BFT consensus algorithm for graph $G$. $G$ must contain a correct $\diamond f+1$-correct-bisource \textbf{and} any subset $V'\subset V$, where $|V'|=n-f$, has fault-free paths in graph $G'=(V,E_{sync})$ to at least $f+1$ correct nodes.

%If there exists a BFT consensus algorithm for graph $G=(V,E)$ then $G$ contains a correct $\diamond f+1$-correct-bisource, \textbf{and} any subset $V'\subset V$, where $|V'|=n-f$, has fault-free paths in graph $G'=(V,E_{sync})$ to at least $f+1$ nodes.

% Existence of CFT algorithm for graph => G has bisource and sync fault-free paths,
% Not existence of CFT algorithm OR G has bisource and sync fault-free paths
%\end{theorem}

\begin{proof}[\textbf{Proof of Theorem \ref{thm:haps-bft-necessary}}]
Suppose for the sake of contradiction there exists a BFT consensus algorithm but the underlying communication graph does not have a $\diamond f+1$-correct-bisource or there exists a subset $V'\subset V$, where $|V'|=n-2f$, has synchronous fault-free paths in graph $G'=(V,E_{sync})$ to at most $f$ nodes.
By theorem \ref{thm:hps-bft-necessary} BFT consensus is not solvable in HPS if there exists a subset $V'\subseteq V-F$, where $|V'|=n-2f$, which is at most $f$-correct-synchronous. Since the adversary in HAPS is strictly more powerful than in HPS this result also applies to HAPS, a contradiction.
By lemma \ref{lem:haps-helper-1} there does not exist a BFT consensus algorithm under HAPS which does not have a $\diamond f+1$-correct-bisource, a contradiction to the assumption. 

%By lemma 1, any subset $V'\subset V$, where $|V'|=n-f$, has fault-free paths in graph $G'=(V,E_{sync})$ to at least $f+1$ nodes. And by lemma 2, $G$ must have a correct $\diamond f+1$-bisource.
\end{proof}

==> disc_2024/async-psync-sync-protocols.tex <==
\section{BFT Consensus Protocols}\label{bft-upper-bounds}
Next, we propose a new consensus algorithm that solves BFT consensus, assuming theorem \ref{thm:hps-bft-necessary} holds. This in turn proves sufficiency of the theorem. We first present the algorithm under HPS, before looking at HAPS.

%In this section, we present a CFT and a BFT consensus protocol for the hybrid asynchrony-partial synchrony-synchrony (HAPS) model. We prove the algorithms correct so long as the adversary maintains the necessary condition from section \ref{}. This proves that the necessary condition is also sufficient.




\subsection{HAPS BFT Consensus Overview}\label{haps-bft-upper-bound}
To prove theorem \ref{thm:haps-bft-necessary} is a sufficient condition, 
%\natacha{To prove thoereom X is sufficient?}\neil{adopted}, 
we propose an algorithm that solves BFT consensus assuming the condition always holds. We could use an off the shelf asynchronous BFT consensus protocol but there are two issues 1) asynchronous BFT consensus protocols are \textbf{not} deterministic and 2) they only work when $n>3f$.
Instead, we adapt our HPS BFT consensus protocol to be resilient to asynchronous edges. Our HPS BFT consensus protocol still maintains safety under HAPS but liveness no longer holds. In HAPS there is no time where all edges behave synchronously (asynchronous edges do not have a $GST$ assumption). Without this assumption, leaders elected in our HPS BFT consensus protocol may continuously timeout, stalling progress. Luckily, we can apply the same trick from the CFT case. The condition from theorem \ref{thm:haps-bft-necessary} guarantees that, when theorem \ref{thm:haps-bft-necessary} holds, there will be a correct $f+1$-correct-bisource. We leverage this correct bisource to guarantee the \textit{no false blame} property. With no false blame, our protocol 1) ensures progress is always made when the correct $f+1$-correct-bisource is elected leader (after GST), and 2) never gets stuck when any other node is elected leader.

%To solve BFT consensus, we devise a protocol that combines techniques from synchronous BFT consensus~\ref{}, partially synchronous BFT consensus protocols like PBFT~\ref{}, and asynchronous BFT consensus protocols like NWH~\ref{} to handle a mixture of synchrony, partial synchrony, and asynchrony. 

%As with our HPS BFT, our HAPS BFT protocol makes use of synchrony to have effectively larger quorums. We know from theorem \ref{} that any set of $n-2f$ honest nodes must be synchronously connected to $f+1$ honest nodes. Since any set of $n-f$ nodes must contain at least $n-2f$ honest nodes, any quorum of $n-f$ effectively contains $f+1$ honest nodes. We take advantage of the quorum intersection property that larger quorums provide to ensure safety despite leader replacements. 

\subsection{HAPS BFT Consensus Utilities}
\par \textbf{Graph Structure.} Our HAPS BFT consensus protocol also uses the $d$ parameter, which is the maximum length of the synchronous fault-free path between any two nodes. Our protocol additionally takes advantage of partially synchronous paths from the correct $f+1$-correct-bisource to prevent spurious view changes. We define $d'$ to be the longest distance of any partially synchronous path in the underlying communication graph. We rely on paramter $d'$ so that nodes wait long enough to retrieve data that is in-flight. If $d'$ is known it can be directly used, otherwise, $d'\coloneqq n-f+1$ to account for the worst case when the longest partially synchronous fault-free path consists of all $n-f$ correct nodes.

%\par \textbf{Protocol Description.}
%Our BFT consensus protocol operates in a series of views, where each view consists of a steady state, and a view change procedure to replace leaders suspected to be faulty. The leader of a view can be elected using a simple round robin scheme (node $v \pmod n$ is the leader of view $v$, where $n$ is the total number of nodes). If the leader fails to send its proposal in a timely fashion, nodes will blame the leader and invoke the view change procedure to replace the leader. After each view change, the view is incremented, and the steady state begins again.

%\par \textbf{Utilities.} Similar to our HPS BFT consensus protocol, nodes \textit{lock} on values that could have been committed. A \textit{lock} consists of a view, value, and $n-f$ \msg{Vote-1}{v,val} messages. It is used to ensure that if a value is committed it will not overwritten by a different value later. Nodes send their locks using a \textsc{Status} message, which also contains the current view. \textsc{HighestRanked} is a procedure that takes in a set of \textsc{Status} messages from at least $n-f$ nodes, and returns the lock with the highest view. This lock is considered to have the highest rank. We use this to preserve safety as the protocol guarantees that if a value is committed then the highest lock must be for that value. 

\subsection{HAPS BFT  Consensus Protocol Details}
\par \textbf{Normal Case.} We first focus on the normal case of the protocol, when progress is made. This guaranteed when the leader of the current view $v$, is a correct node that is $\diamond f+1$-bisource (after GST). The normal case begins when nodes enter view $v$.

\par \underline{\textit{Begin view step.}} Upon entering a new view $v$, a node sends a \msg{Status}{v,lock} to \textbf{all} nodes. When a node receives a set, $S$, containing at least $n-f$ \msg{Status}{v,-} messages, it sends $S$ to all nodes. It then starts a timer for $2d\Delta$ to wait to hear from the leader. When the leader receives the set $S$ containing at least $n-f$ \msg{Status}{v,-} messages, it calls \textsc{HighestRanked} to find the highest rank lock, $val$, if it exists. The leader checks if $val=\bot$. If $val=\bot$, then by quorum intersection no value could have been committed in an earlier view, so the leader can propose its own value, $val_i$. Otherwise if $val\neq \bot$, then the leader must propose $val$ since $val$ could have been committed in an earlier view. The leader sends \msg{Propose}{v,val,S} to all nodes. 

\par \underline{\textit{Equivocation check step.}} If a node receives \msg{Propose}{v,val,S} before its echo timer expires, it proceeds to check whether the leader proposed the correct value. It does so by ensuring $val$ is the highest lock from the set $S$. If so, it begins the checking for equivocation by forwarding the \textsc{Propose} message it received to all nodes. It starts a vote timer for $2d\Delta$, and listens for conflicting \textsc{Propose} messages for a different value in the same view. If it receives a conflicting \textsc{Propose} message for a different value, it detects the leader is faulty and sends a \textsc{Blame} message containing the equivocation, since an honest leader will only send a single \textsc{Propose} message in a view. If the vote timer expires and no conflicting \textsc{Propose} message is received, a node will send a \textsc{Vote-1} message to everybody indicating that it did not detect equivocation. This also ensures it will not send a \textsc{Vote-1} for a different value.

\par \underline{\textit{Locking step.}} When a node receives $n-f$ \msg{Vote-1}{v,val} messages, it forms a lock certificate for $val$. The equivocation check guarantees uniqueness for lock certificates, that is any lock certificate in view $v$ must be for the same value. A node then updates its lock to be the lock certificate for $val$, and then sends a \msg{Vote-2}{v,val} message to all nodes. 

\par \underline{\textit{Commit step.}} Upon receiving $n-f$ \msg{Vote-2}{v,val} messages, a node sends a \msg{Commit}{val} message. Once it receives a \msg{Commit}{val} message it commits $val$, since a quorum of nodes must have locked on $val$. This quorum of nodes will enforce that any future proposed value must be for $val$.


%At a first glance it may seem unnecessary to have both \textsc{Forward-Propose} and \textsc{Vote} messages. The problem with just using \textsc{Vote} messages is that a node can crash in the midst of sending \textsc{Vote} messages to all nodes. This can result in one node receiving a quorum of votes and committing, while other nodes may never receive the committed value before moving to the next view. By multicasting a \textsc{Forward-Propose} message \textit{before} sending a \textsc{Vote} message, we guarantee that even if a node crashes in the process of sending a \textsc{Vote} message to all nodes, it must have sent a message containing the committed value to other nodes. And before moving to the next view, nodes will wait a timeout to receive \textsc{Forward-Propose} messages that were in flight. When a node receives a \msg{Forward-Propose}{v,val} message it updates its local lock to the proposal made by the leader \natacha{Is there a possibility of moving this paragraph after you've finished describing the steady state? It's a bit confusing to have half a conversation}.


\par \textbf{View Change}.
Next, we look at the view change procedure, which replaces leaders when they are suspected faulty. 

\par \underline{\textit{Trigger Conditions.}} The view change is triggered when $n-f$ nodes timeout or detect equivocation. This guarantees that if a correct $f+1$-correct-bisource is the leader, nodes not connected to the bisource cannot initiate view changes by themselves. 

\par \underline{\textit{Waiting Period.}} Upon a node receiving $n-f$ \textsc{Blame} messages (blame certificate), it stops accepting \textsc{Propose} and \textsc{Vote} messages in view $v$ and forwards its lock to all nodes. A node cannot immediately enter the next view but instead must wait $2d\Delta$ before entering the next view. The reason is to give enough time for nodes to receive a lock if some value was committed in the view. If a node does not wait $2d\Delta$ it will miss updating its lock before entering the next view. 

\par \underline{\textit{Enter next view.}} Upon entering the next view, a node sends a \msg{Status}{v,lock} message to all nodes, where $lock$ is the current lock of the node. The normal case then resumes.

\par \textbf{Analysis.} The correctness proofs are found in Appendix \ref{bft-proofs}.

\begin{algorithm}
\begin{algorithmic}[1]
\State{$val_i$}\Comment{The input value of this replica}
\State{$d\gets $ length of longest synchronous fault-free path}
\State{$d'\gets $ length of longest partially synchronous fault-free path}
\State{$v\gets 1$}\Comment{Current view}
%\State{$B_v\gets \bot$}\Comment{Block proposed in current view}
\State{$lock \gets \bot$}\Comment{Highest ranked lock certificate}
\State{$vote\_timer \gets timer(2d\Delta)$}\Comment{Timer for equivocation check}%\Comment{2 Delta is necessary to ensure that there does not exist a fast certificate and a slow certificate for conflicting blocks in the same view}
\State{$echo\_timer \gets timer(2d'\Delta)$}\Comment{Timer for echoing leader value}

\Event{receiving $S\gets n-f$ \msg{Status}{v,-,-} messages}
\State{\textbf{echo} $S$ to all}
\State{\textbf{start} $echo\_timer$}
\State{$//$ \textit{If this node is the leader}}
\If{$i==L_v$}
\State{$val\gets \Call{HighestRank}{S}$}\Comment{Highest (by view) block from all certificates}
\If{$val=\bot$}
\State{$val\gets val_i$}
\EndIf
\State{\textbf{send} \msg{Propose}{v,val,S} to all}\Comment{Leader proposal}
\EndIf
\EndEvent

\Event{receiving \msg{Propose}{v,val,S}}
\If{$val=\Call{HighestRanked}{S} \lor \Call{HighestRank}{S}=\bot$}\Comment{Check leader proposal is valid}
\State{\textbf{echo} \msg{Propose}{v,val,S} to all}\Comment{Echo leader value for equivocation check}
%\State{$val_i\gets val$}\Comment{Current block checking for equivocation}
\State{\textbf{start} $vote\_timer$}\Comment{To detect equivocation}
\EndIf
\EndEvent



%\Event{receiving \msg{Echo}{B,S,v}}
%\State{$C_{v_k}(B_k)\gets \Call{HighestRankedCert}{S}$}
%\If{$B_k\neq B$}\Comment{Proposed block should equal highest ranked certified block}
%\State{\Return}
%\EndIf

%\State{\textbf{forward} \msg{Propose}{B_k,v} to all}
%\State{\textbf{send} \msg{Fast-Vote-1}{B_k,v} to all}%\kartik{do we need to check if it extends the highest block known to me or so?}
%\State{\textbf{start} $vote\_timer$}\Comment{To detect equivocation}
%\EndEvent

%\Event{receiving $FV \gets (n+f+1)/2$ \msg{Fast-Vote-1}{B_k,v}}
%If{$v=v'$}
%State{$FC_{v_f}(B_f) \gets \Call{CreateFastCert}{FV}$}
%\State{$B_{FC} \gets B$}
%State{\textbf{send} \msg{Fast-Vote-2}{FC_v(B_k),v} to all}\Comment{Only vote once per view, block height}
%EndIf
%EndEvent

\Event{$vote\_timer$ expiring and no equivocation}
\State{\textbf{send} \msg{Vote-1}{v,val} to all}
\EndEvent

\Event{receiving $V\gets n-f$ \msg{Vote-1}{v,B}}
\State{$lock\gets (v,val,V)$}\Comment{Lock on this certificate}
\State{\textbf{send} \msg{Vote-2}{v,val} to all}
\EndEvent

%Event{receiving $(n+f+1)/2$ \msg{Fast-Vote-2}{FC_v(B_k),v}}
%State{\textbf{commit} $B_k$ (direct commit) and all ancestors of $B_k$ (indirect commit)}
%State{$B_{\ell}\gets B_k$}
%State{$FC_{v_f}(B_f)\gets FC_v(B_k)$}
%If{$first$}\Comment{After committing first block in view, change to use steady state timer}
%State{$first \gets false$}
%EndIf
%EndEvent

\Event{receiving $n-f$ \msg{Vote-2}{v,val}}
\State{\textbf{send} \msg{Commit}{val} to all}
\EndEvent

\Event{receiving \msg{Commit}{val}}
\State{\textbf{commit} $val$}%\kartik{to myself: why are two rounds of slow votes necessary?}
\EndEvent

\Event{$echo\_timer$ expired $\land$ have not received \msg{Propose}{v,-}}
\State{\textbf{send} \msg{Blame}{v} to all}
\EndEvent

\Event{equivocation detected}
\State{\textbf{forward} equivocation to all}
\State{\textbf{send} \msg{Blame}{v} to all}
\EndEvent

\Event{receiving $BC\gets n-f$ \msg{Blame}{v} messages}
\State{\textbf{forward} $lock$ to all}\Comment{Forward lock certificate to everybody}
\State{\textbf{forward} $BC$ to all}\Comment{Forward blame cert to all}
\State{\textbf{stop} sending \textsc{Vote-1}/\textsc{Vote-2} messages}
\State{\textbf{wait} $2d\Delta$}\Comment{Wait for lock certificate forwarding to finish}
\State{$v\gets v+1$}\Comment{Enter new view}
\State{\textbf{send} \msg{Status}{v,lock} to all}\Comment{Status containing local highest certificate}
\EndEvent

\Event{receiving $lock'=(v',-,-)$}
\State{\textbf{parse} $lock\gets (v,-,-)$}
\If{$v'>v$}
\State{$lock\gets lock'$}\Comment{Update local highest rank cert}
\EndIf

\EndEvent

\end{algorithmic}
\caption{HAPS BFT Consensus Protocol}\label{alg:normal-case}
\end{algorithm}


%Lemma 0: If a fast certificate for $B_l$ forms in view $v$, then any fast certificate that forms in view $v$ must be for $B_l$.
%Proof: A fast certificate requires receiving $2f+1$ \msg{Fast-Vote-2}{B_l,v} messages.
%Lemma $1$: If an honest node directly commits a block $B_l$ in view $v$, then a certified block that ranks no lower than $C_v(B_l)$ must equal or extend $B_l$.

%Proof: A node directly commits block $B_l$ in view $v$ from either 1) receiving $2f+1$ \msg{Fast-Vote-2}{B_l,v} messages or 2) receiving $n-f$ \msg{Slow-Vote-2}{B_l,v} messages. We look at each case individually.

%Case 1) $2f+1$ \msg{Fast-Vote-2}{B_l,v}: Of these $2f+1$ messages, at least $f+1$ of them must have been sent by honest nodes. An honest node only sends a \msg{Fast-Vote-2}{B_l,v} message if it receives $2f+1$ \msg{Fast-Vote-1}{B_l,v} messages, which means $f+1$ honest nodes must have formed a fast certificate for $B_l$. 

==> disc_2024/bft-proofs.tex <==
\section{BFT Consensus Proofs}\label{bft-proofs}

\subsection{HPS BFT Consensus Proofs}



\subsection{HAPS BFT Consensus Proofs}

\par \textbf{Agreement.} The agreement proofs are identical to the HPS BFT case.

\par \textbf{Termination.}
The adversary must let at least one correct $\diamond f+1$-correct-bisource always exist in the underlying communication graph. If there are multiple correct $\diamond f+1$-correct-bisources then let $L_v$ be a correct bisource which remains a correct bisource throughout the execution of the protocol.

\begin{lemma}\label{lem:haps-bft-term-1}
Let view $v$ be the first view after GST for which $L_v$ is elected leader. If no correct node terminates in view $v'<v$, then all correct nodes will reach view $v$.
\end{lemma}

\begin{proof}
We prove the lemma by induction on view $v$.

\par \textbf{Base Case:} $v=1$. All correct nodes start in view $1$, so they reach view $1$ trivially.

\par \textbf{Induction Step.} By the induction assumption we assume no correct node terminates in an earlier view, and all correct nodes reach view $v-1$.

Suppose for the sake of contradiction no correct node terminates in view $v-1$, and at least one correct node never reaches view $v$. If a correct node never reaches view $v$ then it must have never received $n-f$ \msg{Blame}{v-1} messages. 

This implies that at least one correct node never sends a \msg{Blame}{v-1} message. This correct node, $n_1$, must have never received $n-f$ \msg{Blame}{v-1} messages, since $n_1$ would have forwarded the blame certificate to all correct nodes, and they would all eventually advance to view $v$. Instead node $n_1$ must have received a \msg{Propose}{v-1,-,-} message before its echo timer expired (otherwise it would have sent a \msg{Blame}{v-1} message, a contradiction). It then would have echoed the \msg{Propose}{v-1,-,-} message to all nodes, and started its vote timer. It must have sent a \msg{Vote-1}{v-1,-} message to all nodes (otherwise it would have detected equivocation and sent a \msg{Blame}{v-1} message, a contradiction). 

\par We now show that all correct nodes must have sent a \msg{Vote-1}{v-1,-} message. Suppose not, then there must be at least one correct node, $n_2$, which did not send a \msg{Vote-1}{v-1,-} message. Node $n_2$ will eventually receive a \msg{Propose}{v-1,-,-} from node $n_1$. It then will start its vote timer. Since node $n_2$ never sends a \msg{Vote-1}{v-1,-} message, it must have detected equivocation before its vote timer expired. Node $n_2$ will then have forwarded the equivocation to all nodes, which means node $n_1$ must eventually receive the equivocation. Node $n_1$ will then send a \msg{Blame}{v-1} message, a contradiction to the assumption that $n_1$ never sends a \msg{Blame}{v-1} message.

\par Since all correct nodes must have sent a \msg{Vote-1}{v-1,-} message, all correct nodes will eventually receive $n-f$ \msg{Vote-1}{v-1,-} messages. All correct nodes will then send a \msg{Vote-2}{v-1,-} message to all nodes. Therefore, all correct nodes, including node $n_1$ will eventually receive $n-f$ \msg{Vote-2}{v-1,-} messages and commit, a contradiction to the assumption that no correct node terminates in view $v-1$.
\end{proof}

\begin{lemma}\label{lem:haps-bft-term-2}
If all correct nodes enter view $v$, then they all terminate in view $v$.
\end{lemma}

\begin{proof}
When all correct nodes enter view $v$, they send a \textsc{Status} message to all nodes. Thus, all correct nodes will eventually receive $n-f$ \textsc{Status} messages, compute the highest lock and send a \textsc{Forward-HighestRanked} message to all nodes. Any correct node will echo the \textsc{Forward-HighestRanked} message to all nodes (if it has not done so already). Let $B$ be the set of $f+1$ correct nodes which have partially synchronous fault-free paths to $L_v$. Since view $v$ is after GST, and every node in $B$ has a partially synchronous fault-free path to $L_v$, every node in $B$ will receive a \textsc{Propose} message from $L_v$ before their echo timer expires, and forward the \textsc{Propose} message to all nodes for an equivocation check. $L_v$ is correct so it will not equivocate, therefore no node in $B$ will send a \msg{Blame}{v} message. Since a blame certificate requires at least $n-f$ nodes to send a \textsc{Blame} message, and $f+1$ nodes in $B$ will not send a \msg{Blame}{v} message, no blame certificate will ever form in view $v$. Thus eventually all correct nodes will send a \textsc{Vote-1} message, and receive $n-f$ \textsc{Vote-1} messages. Therefore, all correct nodes will send a \textsc{Vote-2} message, and receive $n-f$ \textsc{Vote-2} messages, and terminate in view $v$.
\end{proof}

\begin{theorem}
HAPS BFT satisfies termination.
\end{theorem}

\begin{proof}
If at some point some correct node terminates, it will send a \textsc{Commit} message to all nodes. This message is sent by a correct node, so all correct nodes will eventually receive the message and terminate as well. Now assume that no correct node terminates in any view $v'<v$. In that case by lemma \ref{lem:haps-bft-term-1} all correct nodes eventually reach view $v$. Then by lemma \ref{lem:haps-bft-term-2} all correct nodes terminate during view $v$.
\end{proof}

\par \textbf{Validity.} The validity proof is identical to the HPS BFT case.

%Easy way is to use an off the shelf CFT consensus protocol with n>2f and partially synchronous and then we are done
%the main downside is the replication factor
%if the adversary is a bit weaker can we do better

%The worst case is the adversary corrupts all links
%Unlikely in practice the adversary will corrupt all links to be psync
%We know from section 3 that all
%Necessary condition - Give examples of in practice: for example if n=f+1 then the adversary cannot corrupt any links, if n=2f+1 the adversary can corrupt all links
%HPS is more flexible framework, it aligns
%The next question is does it help, what can we do with it? what is true? is consensus still possible in hps. In sync/psync we understand when consensus is possible or not, our first step is to establish those results for this model
%we can instantiate replication factor bounds depending on the adversary
%give a table of different values

%section 4
%we know consensus is possible in HPS
%we need to design an algorithm that actually
%the obvious strategy, is to use a partially synchronous protocol because in the worst case it psync protocol
%other extreme the adversary corrupts 0 links we know of existing cft sync protocols
%the interesting space is in between the sync and psync extremes
%we're interested in what algorithm we can design for $n<=2f$, for $n>2f$ we can use psync
%add adversary can corrupt up to t paths/links, then in section 3 say
%if cft consensus is solvable then any t links the adversary corrupts such that for all V', V' V' is at least f+1 synchronous
%add a couple of examples to link it back to the t parameter,
%if n=f+1, then any node must have f+1 edges so t must be 0
%if n=2f+1, then f+1 nodes must need at least f+1 sync connections

%show figure examples for synchronous path/k-synchronous, and bisource

==> disc_2024/crash-proofs.tex <==
\section{CFT Consensus Proofs}\label{crash-proofs}
\subsection{HPS CFT Consensus Proofs}



\subsection{HAPS CFT Consensus Proofs}

\par \textbf{Agreement.} The agreement proofs are identical to the HPS CFT case.

%\begin{lemma}\label{lem:haps-cft-1}
%If a node receives a \msg{Commit}{val} message in view $v$, then at least $f+1$ nodes will set $lock\gets (v,val)$ before exiting view $v$.
%\end{lemma}

%\begin{proof}
%If a node received a \msg{Commit}{val} message in view $v$ then at least $n-f$ nodes have sent a \msg{Vote}{v,val} message. Let $P$ be this set of $n-f$ nodes which sent a \msg{Vote}{v,val} message. By theorem \ref{thm:haps-cft-necessary} any set of $n-f$ nodes must have synchronous fault-free paths to at least $f+1$ distinct nodes. Let $Q$ be this set of $f+1$ nodes. We now show that every node $q\in Q$ sets its $lock=(v,val)$ before exiting view $v$. Since the graph is undirected, node $q$ must have a synchronous fault-free path to at least one node, $p\in P$. Let $t_q$ be the time node $q$ sends a \msg{Blame}{v} message. This message is sent to all nodes, which node $q$ will receive by time $t_q+d\Delta$, where $d$ is the distance of the longest synchronous fault-free path. There are two cases: 1) node $p$ has sent a \msg{Vote}{v,val} message before time $t_q+d\Delta$ or 2) node $p$ has sent a \msg{Vote}{v,val} message after time $t_q+d\Delta$.


%\textbf{Case 1.} Node $p$ sent a \msg{Vote}{v,val} message to all nodes before time $t_q+d\Delta$. Before sending a \msg{Vote}{v,val} message, node $p$ must have sent a \msg{Forward-Propose}{v,val} message to all nodes. Since node $p$ has a synchronous fault-free path to node $q$, and this \textsc{Forward-Propose} message is echoed, node $q$ will receive \msg{Forward-Propose}{v,val} by time $t_q+2d\Delta$. Since $q$ waits $2d\Delta$ time after sending a \msg{Blame}{v} message before moving to view $v+1$, it must have received \msg{Forward-Propose}{v,val}, and updated its $lock=(v,val)$ before exiting view $v$.


%\textbf{Case 2.} Node $p$ sent a \msg{Vote}{v,val} message to all nodes after time $t_q+d\Delta$. Node $p$ received a \msg{Blame}{v} message by time $t_q+d\Delta$. Once it receives a \textsc{Blame} message it does not accept any \textsc{Propose} messages in view $v$, and therefore does not send a \textsc{Vote} message in view $v$. This is a contradiction, so node $p$ must have sent \msg{Vote}{v,val} before time $t_q+d\Delta$.


%We showed that every node $q\in Q$ will update $lock\gets (v,val)$ before exiting view $v$. Since $|Q|$ is at least $f+1$, the lemma is satisfied.
%\end{proof} 


%\begin{lemma}\label{lem:haps-cft-3}
%If some node receives a \msg{Commit}{commit\_val} in view $v$, then any \msg{Propose}{v',val} message in view $v'>v$ must have $val=commit\_val$.
%\end{lemma}

%\begin{proof}
%We prove this by induction. 

%\par \textbf{Base case: $v'=v+1$.} By lemma \ref{lem:hps-cft-1} at least $f+1$ nodes will set $lock=(v,val)$ before exiting view $v$. If the leader of view $v'$ sends a \msg{Propose}{v',val} message, then it must have received a set of $n-f$ \msg{Status}{v',val} messages. By quorum intersection, at least one of these \textsc{Status} messages must have $lock=(v,val)$. Since $v=v'-1$ is the highest possible view for a lock, and $val$ is the only possible proposed value in $v$, \textsc{HighestRanked} must return $val$. Therefore, any \msg{Propose}{v+1,val'} message, must have $val'=val$.

%\par \textbf{Induction Step: $v'-1>v$} We assume the lemma holds for all $v'-1>v$, and now we consider view $v'$. If the leader of $v'$ sends a \textsc{Propose} message, then the leader of $v'$ must have received a set $S$ containing $n-f$ \msg{Status}{v',lock} messages. By lemma \ref{lem:haps-cft-1} there are at least $f+1$ nodes which have set $lock=(v,val)$. By the induction assumption any \textsc{Propose} message for any view between $v$ and $v'-1$ must be for $val$. Therefore, at least $f+1$ nodes will have $lock=(v'',val)$, where $v\leq v''\leq v'-1$. By quorum intersection, any set of $n-f$ \textsc{Status} messages must contain at least one $lock=(v'',val)$, where $v''\geq v$. \textsc{HighestRanked}($S$) therefore must return $val$, and so any \msg{Propose}{v',val'} message must have $val'=val$.
%\end{proof}

%\begin{theorem}
%Any two nodes will commit the same value.    
%\end{theorem}

%\begin{proof}
%Let $v$ be the earliest view in which a node commits some value, $val$. Any other node will either commit in 1) view $v$ or 2) view $v'>v$. If a node commits in view $v$, then it must also commit $val$, since another node committed $val$ in view $v$ any \textsc{Propose} message for view $v$ must be for $val$. If a node commits in view $v'>v$, then by lemma \ref{lem:haps-cft-3} any \msg{Propose}{v',val'} message must have $val'=val$. Therefore it will also decide $val$. In both cases nodes will commit the same value, satisfying the theorem.
%\end{proof}

\par \textbf{Termination.} The adversary must let at least one correct $\diamond f+1$-bisource always exist in the underlying communication graph. If there are multiple correct $\diamond f+1$ bisources, then let $L_v$ be a correct bisource that remains a correct bisource throughout the execution of the protocol. $L_v$ will be elected leader infinitely often (by the round-robin leader election scheme).

\begin{lemma}\label{lem:haps-cft-term-1}
If a correct node never reaches view $v$, then at least one correct node never sends a \msg{Blame}{v-1} message.
\end{lemma}

\begin{proof}
Suppose for the sake of contradiction a correct node, $n_1$, never reaches view $v$, and all correct nodes send a \msg{Blame}{v-1} message. Eventually, all correct nodes (including node $n_1$) will receive $n-f$ \msg{Blame}{v-1} messages. Node $n_1$ will send and receive a \msg{Blame-Cert}{v-1} message, and then enter view $v$ after $2d\Delta$ time, a contradiction.
\end{proof}

\begin{lemma}\label{lem:haps-cft-term-2}
If a correct node, $n_1$, never sends a \msg{Blame}{v-1} message then either all correct nodes will send a \msg{Vote}{v,-} message in view $v$ or $n_1$ will receive a \msg{Blame-Cert}{v-1} message.   
\end{lemma}

\begin{proof}
Suppose for the sake of contradiction node $n_1$ never sends a \msg{Blame}{v-1} message, never reaches view $v$, and there is at least one correct node, $n_2$, which never sends a \msg{Vote}{v,-} message in view $v$. Since node $n_1$ never sends a \msg{Blame}{v-1} message, it must have received a \msg{Propose}{v-1,-} message, and echoed it to all nodes (including node $n_2$). Node $n_2$ will thus eventually receive a \msg{Propose}{v-1,-} message from node $n_1$. If node $n_2$ does not process the \msg{Propose}{v-1,-} message it must have sent a \msg{Blame-Cert}{v-1} message to all nodes. Node $n_1$ will eventually receive this message, a contradiction. Otherwise, node $n_2$ will process the \msg{Propose}{v-1,-} message, update its lock, and send a \msg{Vote}{v,-} message to all nodes, a contradiction. 
\end{proof}


\begin{lemma}\label{lem:haps-cft-term-3}
Let $v$ be the first view after GST for which $L_v$ is elected leader. If no correct node terminates in view $v'<v$, then all correct nodes will reach view $v$.
\end{lemma}

\begin{proof}
We prove the lemma by induction on view $v$.
\par \textbf{Base Case: $v=1$.} All correct nodes start in view $1$, so they reach view $1$ trivially.
\par \textbf{Induction Step.} By the induction assumption, we assume no correct node terminates in an earlier view, and all correct nodes reach view $v-1$.

Suppose for the sake of contradiction no correct node terminates in view $v-1$, and at least one correct node, $n_1$ never reaches view $v$. 

By lemma \ref{lem:haps-cft-term-1}, there must be at least one correct node which never sends a \msg{Blame}{v-1} message. Let this node be $n_2$. By lemma \ref{lem:haps-cft-term-2}, either node $n_2$ will receive a \msg{Blame-Cert}{v-1} message or all correct nodes will send a \msg{Vote}{v-1,-} message. If node $n_2$ receives a \msg{Blame-Cert}{v-1} message, it will echo it to all nodes (including node $n_1$), therefore node $n_1$ will eventually receive it and enter view $v$ after $2d\Delta$ time, a contradiction. Otherwise, all correct nodes must have sent \msg{Vote}{v-1,-}, and therefore all correct nodes will eventually receive $n-f$ \msg{Vote}{v-1,-} messages (since there are $n-f$ correct nodes), and send a \textsc{Commit} message to all nodes. This will cause all correct nodes to eventually terminate in view $v-1$, a contradiction to the assumption that no correct node terminates in view $v-1$.


%If a correct node never reaches view $v$ then it must never receive a \msg{Blame-Cert}{v-1} message (otherwise it would advance to view $v$).

%This implies that at least one correct node never sends a \msg{Blame}{v-1} message. This correct node, $n_1$, must have never received $n-f$ \msg{Blame}{v-1} messages (otherwise it would have sent a \msg{Blame-Cert}{v-1} message to all nodes, a contradiction). Instead node $n_1$ must have received a \msg{Propose}{v-1,-} message, and sent a \textsc{Forward-Propose} and \textsc{Vote-1} message to all nodes.


%We now show that all correct nodes must have sent a \msg{Vote}{v-1,-} message. Suppose not, then there must be at least one correct node, $n_2$, which did not send a \msg{Vote}{v-1,-} message. If node $n_2$ received a \msg{Blame-Cert}{v-1} message, it will echo the message to all nodes, including node $n_1$, causing node $n_1$ to eventually advance to view $v$, a contradiction. Therefore, node $n_2$ could not have received a \msg{Blame-Cert}{v-1} message. Node $n_2$ instead will eventually receive a \msg{Propose}{v-1,-} message from node $n_1$, and process it because it never receives a \msg{Blame-Cert}{v-1} message. This will cause node $n_2$ to send a \textsc{Forward-Propose} and \textsc{Vote} message, a contradiction.


%Since all correct nodes must have sent a \msg{Vote}{v-1,-} message, all correct nodes will eventually receive $n-f$ \msg{Vote}{v-1,-} messages and commit, a contradiction to the assumption that no correct node terminates in view $v-1$.
\end{proof}

\begin{lemma}\label{lem:haps-cft-term-4}
If all correct nodes enter view $v$, then they all terminate in view $v$.
\end{lemma}

\begin{proof}
When all correct nodes enter view $v$, they send a \textsc{Status} message to all nodes. Thus, all correct nodes will eventually receive $n-f$ \textsc{Status} messages, compute the highest lock, and send a \textsc{Forward-HighestRanked} message to all nodes. Any correct node will echo a \textsc{Forward-HighestRanked} message to all nodes (if it has not done so already). Let $B$ be the set of $f+1$ nodes which have partially synchronous fault-free paths to $L_v$. Since view $v$ is after GST, and every node in $B$ has a partially synchronous fault-free path to $L_v$, every node in $B$ will receive a \textsc{Propose} message from $L_v$ before their echo timer expires. Thus, no node in $B$ will send a \msg{Blame}{v} message. Since a blame certificate requires $n-f$ nodes to send a \textsc{Blame} message, and $f+1$ nodes in $B$ will not send a \msg{Blame}{v} message, no blame certificate will ever form in view $v$. Thus all correct nodes will eventually receive a \textsc{Propose} message, update their local $lock$, and send a \msg{Vote}{v,-} message to all nodes. All correct nodes will eventually receive $n-f$ \msg{Vote}{v,-} messages and terminate in view $v$.
\end{proof}

\begin{theorem}
All correct nodes eventually terminate.    
\end{theorem}

\begin{proof}
If at some point some correct node terminates, it will send a \textsc{Commit} message to all nodes. This message is sent by a correct node, so all correct nodes will eventually receive the \textsc{Commit} message and terminate as well. Now assume that no correct node terminates in any view $v'<v$. In that case by lemma \ref{lem:haps-cft-term-3}, all correct nodes will eventually reach view $v$. Then by lemma \ref{lem:haps-cft-term-4}, all correct nodes terminate during view $v$.
\end{proof}

\par \textbf{Validity.} The validity proof is identical to the HPS CFT case.
%\begin{theorem}
%Any decided proposal is the input value of some node    
%\end{theorem}

%\begin{proof}
%Nodes only decide if they receive \msg{Commit}{val} message. The value, $val$, in a \textsc{Commit} message must have been proposed by a leader. Since a leader must either propose its own input value or a value proposed by an earlier leader, $val$ must be the input value of some node.
%\end{proof}


==> disc_2024/psync-async-sync-cft.tex <==





\section{CFT Consensus under HAPS}\label{s:cft-necessary}


\begin{theorem}\label{thm:haps-cft-necessary}
Under fine-grained synchrony with asynchrony, CFT consensus with $n\leq 2f$ is solvable if and only if: (i) for all set $A$ of $n-f$ nodes, there exists a set $B$ of at least $f+1$ nodes such that $A \rightarrow B$, and (ii) there is at least one node that is a correct $f+1$ bisource.
\end{theorem}
\rl{meaning that one node is correct or it is connected to f+1 correct nodes?} 

In HPS \textit{every edge} is guaranteed to be at least eventually synchronous, whereas HAPS allows for some edges to remain asynchronous. Solving consensus determistically in HAPS thus requires additional synchrony assumptions to circumvent FLP. Specifically, the minimum requirement is a correct node with partially synchronous connections to at least $f+1$ nodes, or a correct $\diamond f+1$-bisource. \rl{cite or credit the other paper somewhere?}

Intuitively, without a correct $\diamond f+1$-bisource, each leader is partially connected to at most $f$ nodes.
The other $n-f$ nodes cannot tell whether those $f$ nodes (including the leader) are faulty or slow. 
Therefore, no leader can provide liveness to the protocol. 


\subsection{Necessity}\label{s:haps-cft-necessary}
Next we prove that theorem \ref{thm:haps-cft-necessary} is a necessary condition for solving consensus under HAPS.

\rl{to be updated}

%A correct $\diamond f+1$-bisource ensures that at least $f+1$ nodes will eventually have synchronous communication with each other by using the correct bisource as a router. These $f+1$ nodes can eventually reach agreement using a simple synchronous protocol, and then broadcast their decision to all other nodes. Of these $f+1$ nodes, at least one must be correct, so all other nodes will eventually receive the decision value.
%\natacha{Given you're doing necessary here rather than sufficiency, it'd be great to reformulate the intuition as more of why it will be broken "unless". Having said that, I think it's great intuition for explaining 3.1. The current text also makes it sound like solving th eproblem in HAPS is "easier" than HPS. It also doesn't really discuss randomness}

\begin{lemma}\label{lem:haps-cft-bisource}
If there exists a CFT consensus algorithm under the HAPS model tolerating at most $f$ crash faulty nodes and $s$ link alterations, then there must exist a correct $\diamond f+1$-bisource in the underlying communication graph.

%There does not exist a CFT consensus algorithm in HAPS which does not contain a correct $\diamond f+1$-bisource.

\end{lemma}

\begin{proof}
Suppose for the sake of contradiction there exists an algorithm, $A$, which solves CFT consensus under HAPS when the underlying communication graph does not have a correct $\diamond f+1$-bisource. We show how to solve consensus in full asynchrony with one crash failure using this CFT consensus algorithm, which contradicts the FLP result that this is impossible. 


Consider a set, $P$, of $n-f+1$ nodes, of which one node is faulty, and there are only asynchronous links between nodes. We construct a communication graph, $G_1$, which contains $P$ and a set, $Q$, of $f-1$ faulty dummy nodes. The adversary changes all links between nodes in $P$ to be asynchronous. The rest of the links remain synchronous. As every node in $P$ only has synchronous links to nodes in $Q$, and $|Q|=f-1$, there does not exist a correct $\diamond f+1$-bisource.


By assumption, there must exist an algorithm, $A$, that solves CFT consensus even when the adversary changes links so that there does not exist a correct $\diamond f+1$-bisource. We now show that one can solve CFT consensus among nodes in $P$ ($P$ has one crash faulty node) in a fully asynchronous network. To solve consensus among nodes in $P$, nodes in $P$ just execute $A$ pretending that the communication graph is $G_1$, where $Q$ is just a set of dummy nodes that have crashed from the beginning. Note that in $G_1$ all links between nodes in $P$ are asynchronous. $A$ therefore solves CFT consensus in an asynchronous network with one crash failure, a contradiction to the FLP result~\cite{flp}. 
\end{proof}

%\begin{theorem}
%If CFT consensus is solvable in HAPS, then the underlying communication graph must always have a correct $\diamond f+1$-bisource, \textbf{and} $\forall V'\in {V \choose n-f}$, $V'$ must be at least $f+1$-synchronous.
%\end{theorem}

\begin{proof}[\textbf{Proof of Theorem \ref{thm:haps-cft-necessary}}]
%By lemma 1, any subset $V'\subset V$, where $|V'|=n-f$, has fault-free paths in graph $G'=(V,E_{sync})$ to at least $f+1$ nodes. And by lemma 2, $G$ must have a correct $\diamond f+1$-bisource.

Suppose for the sake of contradiction CFT consensus is solvable in HAPS but the underlying communication graph does not contain a correct $\diamond f+1$-bisource \textbf{or} there exists a subset $V'\subseteq V$, where $|V'|=n-f$ nodes, and $V'$ is at most $f$-synchronous.

By theorem \ref{thm:hps-cft-necessary}, CFT consensus is not solvable in HPS if there exists a subset $V'\subseteq V$, where $|V'|=n-f$ nodes, which is at most $f$-synchronous. Since the adversary in HAPS is strictly more powerful than in HPS this result also applies to HAPS, a contradiction to the assumption. By lemma \ref{lem:haps-cft-bisource}, there does not exist a CFT consensus algorithm under HAPS for a graph which does not contain a correct $\diamond f+1$-bisource, a contradiction to the assumption.
\end{proof}


\subsection{Protocol Overview}

Our HPS CFT protocol still maintains safety under HAPS but will lose liveness because no leader can reach all nodes in time.
We need to modify the protocol to leverage the $f+1$-bisource node for liveness. 

In particular, we need to make sure that the bisource node is not falsely removed after GST. 
To achieve this property, we require $n-f$ (instead of one) blame messages to trigger a view change. 
Since the $f+1$ partially connected nodes will not blame the bisource leader, the leader can ensure termination in its view. 


\rl{protocol is similar to last one, move details to appendix. Also, let's not repeat the whole thing, just highlight the diff}

\par \underline{\textit{Begin view step.}}
Upon entering a new view $v$, a node sends a \msg{Status}{v,lock} message to \textbf{all} nodes (Alg. \ref{alg:cft-haps} line \ref{status-haps}). %\natacha{Still to present tense? all nodes broadcasts, eventually, a node receives, etc. Changed it for you already} 
When a node eventually receives at least $n-f$ \msg{Status}{v,-} messages, it calls \textsc{HighestRanked} to find the highest ranked lock from these set of \textsc{Status} messages (Alg. \ref{alg:cft-haps} line \ref{highest-rank-haps}). It then includes this lock in the \textsc{Forward-HighestRanked} message it sends to all nodes (Alg. \ref{alg:cft-haps} line \ref{forward-high-rank}). The node then starts a timer with $2d'\Delta$ duration (Alg. \ref{alg:cft-haps} line \ref{start-echo-timer-haps}). This timer duration ensures that if the leader is a correct $\diamond f+1$-bisource, then all nodes will receive its proposal before its echo timer expires.
%\natacha{Can you make sure to corresponding pseudo code lines? It's a lot to read a full block of text like this}

\par \underline{\textit{Leader proposal step.}} Upon receiving a \msg{Forward-HighestRanked}{v,val} message, the leader checks if $val=\bot$. If $val=\bot$, then no value could have been committed in an earlier view (by quorum intersection any committed value must be the highest ranked value), so the leader can propose its own value, $val_i$. Otherwise if $val\neq \bot$, then the leader must propose $val$ since $val$ could have been committed in an earlier view (Alg. \ref{alg:cft-haps} lines \ref{check-high-rank-haps}-\ref{end-check-high-rank-haps}). The leader sends a \msg{Propose}{v,val} to all nodes (Alg. \ref{alg:cft-haps} line \ref{send-leader-prop-haps}). 

\par \underline{\textit{Receive proposal step.}} In the good case, a node will receive a \msg{Propose}{v,val} message from the leader before its $echo\_timer$ expires. Upon receiving \msg{Propose}{v,val}, the node echoes the \textsc{Propose} message and updates its local $lock=(v,val)$ (Alg. \ref{alg:cft-haps} line \ref{update-lock-haps}). After a node updates its lock, it will \textbf{first} send a \msg{Forward-Propose}{v,val} to all nodes \textit{before} sending a \msg{Vote}{v,val} message to all nodes (Alg. \ref{alg:cft-haps} lines \ref{forward-prop-haps}-\ref{vote-send-haps}). The \textsc{Forward-Propose} message is sent to propagate the leader's proposal to more nodes. 


%At a first glance it may seem unnecessary to have both \textsc{Forward-Propose} and \textsc{Vote} messages. The problem with just using \textsc{Vote} messages is that a node can crash in the midst of sending \textsc{Vote} messages to all nodes. This can result in one node receiving a quorum of votes and committing, while other nodes may never receive the committed value before moving to the next view. By sending a \textsc{Forward-Propose} message \textit{before} sending a \textsc{Vote} message, we guarantee that even if a node crashes in the process of sending a \textsc{Vote} message to all nodes, it must have sent a message containing the committed value to other nodes. And before moving to the next view, nodes will wait enough time to receive \textsc{Forward-Propose} messages that were in flight. When a node receives a \msg{Forward-Propose}{v,val} message it updates its local lock to the proposal made by the leader \natacha{Is there a possibility of moving this paragraph after you've finished describing the steady state? It's a bit confusing to have half a conversation}.
\par \underline{\textit{Echo proposal step.}} When a node receives a \msg{Forward-Propose}{v,val} message, it updates its local $lock=(v,val)$, and then forwards the \msg{Forward-Propose}{v,val} message to all nodes (Alg. \ref{alg:cft-haps} line \ref{echo-forward-pop-haps}). This echo step is necessary to have the leader's proposal reach at least $f+1$ nodes.

\par \underline{\textit{Commit step.}} When a node receives a quorum of $n-f$ \msg{Vote}{v,val} messages it sends a \msg{Commit}{val} message to all (Alg. \ref{alg:cft-haps} line \ref{send-commit-haps}). Upon receiving a \msg{Commit}{val} message it commits $val$ (Alg. \ref{alg:cft-haps} line \ref{receive-commit-haps}).


\par \textbf{View Change}. 
%\natacha{Is there any chance you could add some structure to the next? Right now it's a wall of text so hard to follow each step?} 
%When the elected leader is not the correct $\diamond f+1$-bisource its proposal may not reach all the nodes. We therefore have a view change protocol that is triggered when at least $n-f$ nodes, suspect the leader is not the correct $\diamond f+1$-bisource or it is before GST and the links of the bisource are not synchronous yet. A quorum of $n-f$ nodes ensures that at least one of the nodes (by quorum intersection) must be one of the $f+1$ nodes that the bisource has partially synchronous links to. This prevents a spurious view change of the correct $\diamond f+1$-bisource after GST.
We have a view change procedure that replaces leaders when they are suspected faulty.


\par \underline{\textit{Trigger Conditions.}} A node suspects the leader is faulty if it does not receive a \msg{Propose}{v,-} message before its echo timer expires. When this occurs, a node then sends a \textsc{Blame} message to all nodes, indicating it wishes to quit the view (Alg. \ref{alg:cft-haps} line \ref{send-blame-haps}). When a node receives $n-f$ \textsc{Blame} messages for the current view, it sends a \textsc{Blame-Cert} message to all nodes (Alg. \ref{alg:cft-haps} line \ref{forward-blame-cert-haps}). Once a node receives a \textsc{Blame-Cert} message, it begins the waiting period.

\par \underline{\textit{Waiting Period.}} When a node receives a \textsc{Blame-Cert} message for the current view, it forwards the message to all nodes, so other nodes will also quit the current view (Alg. \ref{alg:cft-haps} line \ref{forward-blame-cert-haps}). Afterwards, the node waits $2d\Delta$ before moving on to the next view (Alg. \ref{alg:cft-haps} line \ref{wait-period-haps}). During this waiting period, the node will stop accepting \textsc{Propose} messages, and listen for \textsc{Forward-Propose} messages that may have just been sent (Alg. \ref{alg:cft-haps} line \ref{stop-prop-haps}). The waiting period is necessary to ensure that a node will not miss updating its lock before entering the next view.

\par \underline{\textit{Enter next view.}} After the waiting period is over, a node can safely move to the next view (Alg. \ref{alg:cft-haps} line \ref{new-view-haps}). The normal case then resumes.





%When a node receives a \msg{Blame-Cert}{v} message, it forwards this message to all. The \msg{Blame-Cert}{v} message is a ticket for nodes to know they should move on to the next view. However, a node cannot just move to the next view immediately. The reason is that another node may have simultaneously sent a \msg{Vote}{v,val} message. A node that view changes may miss receiving the \msg{Forward-Propose}{v,val} message before entering the next view. This can violate safety, as if $val$ is committed then we need at least $f+1$ nodes to lock on $(v,val)$ before exiting the view. A node thus waits $2d\Delta$ before entering the next view to receive a \textsc{Forward-Propose} message that is in-flight. Upon entering the next view, a node returns to the steady state.

%\par \textbf{Analysis.} The correctness proofs are found in Appendix \S\ref{crash-proofs}.

% The reason is that suppose a node in the synchronous connected subgraph receives a \msg{Blame-Cert}{v} message at time $t$. \msg{Blame-Cert}{v} will be received by all nodes in the synchronous connected subgraph by time $t+d\Delta$. This is the latest time a node can send a \msg{Vote}{v,val} message because upon receiving a \msg{Blame-Cert}{v} message a node stops processing \textsc{Propose} messages. We know that the node could at the latest have sent a \msg{Forward-Propose}{v,val} message at time $t+d\Delta$. So since the \msg{Forward-Propose}{v,val} message is multi-casted at time $t+d\Delta$ it is guaranteed to reach all nodes in the synchronous connected subgraph by time $t+2d\Delta$. By waiting $2d\Delta$ before entering the next view, we guarantee that nodes in the synchronous connected subgraph have enough time to process \textsc{Forward-Propose} messages before exiting the view. Upon entering the next view, a node returns to the steady state.

\begin{algorithm}
\begin{algorithmic}[1]
\State{$d\gets $ length of the longest synchronous fault-free path}
\State{$d'\gets $ length of longest partially synchronous fault-free path}
%\State{$val_i$}\Comment{The input value of this replica}
%\State{$v\gets 1$}\Comment{Current view}
\State{$v_i\gets 1$}
\State{$lock \gets \bot$}\Comment{Highest ranked slow certificate}
%\State{\textbf{enter} view 1}

\State{$echo\_timer \gets timer(2d'\Delta)$}\Comment{Timer for receiving leader value}

\Event{receiving $S\gets n-f$ \msg{Status}{v,-} messages}
\State{$val \gets \Call{HighestRanked}{S}$}\label{highest-rank-haps}
%\State{\textbf{send} \msg{Forward-HighestRanked}{v,val} to all}
\State{\textbf{echo} $S$ to all}\label{forward-high-rank}
\State{\textbf{start} $echo\_timer$}\label{start-echo-timer-haps}

\If{$i=L_v$}
\If{$val=\bot$}\label{check-high-rank-haps}
\State{$val\gets val_i$}\Comment{Propose current input value}
\EndIf\label{end-check-high-rank-haps}
\State{\textbf{send} \msg{Propose}{v,val} to all}\Comment{Leader proposal}\label{send-leader-prop-haps}
\EndIf
\EndEvent


\Event{receiving \msg{Propose}{v,val}}
\State{$lock \gets (v,val)$}\label{update-lock-haps}
\State{\textbf{echo} \msg{Propose}{v,val} to all}
%\State{\textbf{send} \msg{Forward-Propose}{v,val} to all}\label{forward-prop-haps}
\State{\textbf{send} \msg{Vote}{v,val} to all}\label{vote-send-haps}
\EndEvent

\Event{receiving $n-f$ \msg{Vote}{v,val}}
\State{\textbf{send} \msg{Commit}{val} to all}\label{send-commit-haps}
\EndEvent

\Event{receiving \msg{Commit}{val}}
\State{\textbf{commit} $val$}\label{receive-commit-haps}
\EndEvent

\Event{$echo\_timer$ expiring and have not received \msg{Propose}{v,-}}
\State{\textbf{send} \msg{Blame}{v} to all}\label{send-blame-haps}
\EndEvent

\Event{receiving $n-f$ \msg{Blame}{v'}, where $v'\geq v$}
\State{\textbf{send} \msg{Blame-Cert}{v} to all}\label{send-blame-cert-haps}
\EndEvent

\Event{receiving \msg{Blame-Cert}{v'}, where $v'\geq v$}
\State{\textbf{echo} \msg{Blame-Cert}{v'} to all}\label{forward-blame-cert-haps}
\State{\textbf{wait} $2d\Delta$}\Comment{Wait for Forward-Propose messages to propagate to all replicas in the connected component}\label{wait-period-haps}
\State{\textbf{stop} accepting \textsc{Propose}, do not send \textsc{Vote} messages in view $v'$}\label{stop-prop-haps}
\State{$v\gets v'+1$}\label{new-view-haps}
\State{\textbf{send} \msg{Status}{v,lock} to all}\label{status-haps}
\EndEvent

\end{algorithmic}
\caption{HAPS CFT Consensus Protocol}\label{alg:cft-haps}
\end{algorithm}

\subsection{Analysis}

\begin{theorem} (Agreement)
No two nodes commit different values.    
\end{theorem}

\begin{proof}
Same proof as \gps{}.
\end{proof}

%\par \textbf{Agreement.} The agreement proofs are identical to the \gps{} CFT case.

%\par \textbf{Termination.} 
%Let $L_v$ be a correct node inside the largest connected component that remains a correct bisource throughout the execution of the protocol. $L_v$ will be elected leader infinitely often (by the round-robin leader election scheme).

\begin{lemma}\label{lem:haps-cft-term-1}
If a correct node never reaches view $v$, then at least one correct node never sends a \msg{Blame}{v-1} message.
\end{lemma}

\begin{proof}
Suppose for the sake of contradiction a correct node, $n_1$, never reaches view $v$, and all correct nodes send a \msg{Blame}{v-1} message. Eventually, all correct nodes (including node $n_1$) will receive $n-f$ \msg{Blame}{v-1} messages. Node $n_1$ will send and receive a \msg{Blame-Cert}{v-1} message, and then enter view $v$ after $2d\Delta$ time, a contradiction.
\end{proof}

\begin{lemma}\label{lem:haps-cft-term-2}
If a correct node, $n_1$, never sends a \msg{Blame}{v-1} message then either all correct nodes will send a \msg{Vote}{v,-} message in view $v$ or $n_1$ will receive a \msg{Blame-Cert}{v-1} message.   
\end{lemma}

\begin{proof}
Suppose for the sake of contradiction node $n_1$ never sends a \msg{Blame}{v-1} message, never reaches view $v$, and there is at least one correct node, $n_2$, which never sends a \msg{Vote}{v,-} message in view $v$. Since node $n_1$ never sends a \msg{Blame}{v-1} message, it must have received a \msg{Propose}{v-1,-} message, and echoed it to all nodes (including node $n_2$). Node $n_2$ will thus eventually receive a \msg{Propose}{v-1,-} message from node $n_1$. If node $n_2$ does not process the \msg{Propose}{v-1,-} message it must have sent a \msg{Blame-Cert}{v-1} message to all nodes. Node $n_1$ will eventually receive this message, a contradiction. Otherwise, node $n_2$ will process the \msg{Propose}{v-1,-} message, update its lock, and send a \msg{Vote}{v,-} message to all nodes, a contradiction. 
\end{proof}


\begin{lemma}\label{lem:haps-cft-term-3}
Let $v$ be the first view after GST for which $L_v$ is elected leader. If no correct node terminates in view $v'<v$, then all correct nodes will reach view $v$.
\end{lemma}

\begin{proof}
We prove the lemma by induction on view $v$.
\par \textbf{Base Case: $v=1$.} All correct nodes start in view $1$, so they reach view $1$ trivially.
\par \textbf{Induction Step.} By the induction assumption, we assume no correct node terminates in an earlier view, and all correct nodes reach view $v-1$.

Suppose for the sake of contradiction no correct node terminates in view $v-1$, and at least one correct node, $n_1$ never reaches view $v$. 

By lemma \ref{lem:haps-cft-term-1}, there must be at least one correct node which never sends a \msg{Blame}{v-1} message. Let this node be $n_2$. By lemma \ref{lem:haps-cft-term-2}, either node $n_2$ will receive a \msg{Blame-Cert}{v-1} message or all correct nodes will send a \msg{Vote}{v-1,-} message. If node $n_2$ receives a \msg{Blame-Cert}{v-1} message, it will echo it to all nodes (including node $n_1$), therefore node $n_1$ will eventually receive it and enter view $v$ after $2d\Delta$ time, a contradiction. Otherwise, all correct nodes must have sent \msg{Vote}{v-1,-}, and therefore all correct nodes will eventually receive $n-f$ \msg{Vote}{v-1,-} messages (since there are $n-f$ correct nodes), and send a \textsc{Commit} message to all nodes. This will cause all correct nodes to eventually terminate in view $v-1$, a contradiction to the assumption that no correct node terminates in view $v-1$.


%If a correct node never reaches view $v$ then it must never receive a \msg{Blame-Cert}{v-1} message (otherwise it would advance to view $v$).

%This implies that at least one correct node never sends a \msg{Blame}{v-1} message. This correct node, $n_1$, must have never received $n-f$ \msg{Blame}{v-1} messages (otherwise it would have sent a \msg{Blame-Cert}{v-1} message to all nodes, a contradiction). Instead node $n_1$ must have received a \msg{Propose}{v-1,-} message, and sent a \textsc{Forward-Propose} and \textsc{Vote-1} message to all nodes.


%We now show that all correct nodes must have sent a \msg{Vote}{v-1,-} message. Suppose not, then there must be at least one correct node, $n_2$, which did not send a \msg{Vote}{v-1,-} message. If node $n_2$ received a \msg{Blame-Cert}{v-1} message, it will echo the message to all nodes, including node $n_1$, causing node $n_1$ to eventually advance to view $v$, a contradiction. Therefore, node $n_2$ could not have received a \msg{Blame-Cert}{v-1} message. Node $n_2$ instead will eventually receive a \msg{Propose}{v-1,-} message from node $n_1$, and process it because it never receives a \msg{Blame-Cert}{v-1} message. This will cause node $n_2$ to send a \textsc{Forward-Propose} and \textsc{Vote} message, a contradiction.


%Since all correct nodes must have sent a \msg{Vote}{v-1,-} message, all correct nodes will eventually receive $n-f$ \msg{Vote}{v-1,-} messages and commit, a contradiction to the assumption that no correct node terminates in view $v-1$.
\end{proof}

\begin{lemma}\label{lem:haps-cft-term-4}
If all correct nodes enter view $v$, then they all terminate in view $v$.
\end{lemma}

\begin{proof}
When all correct nodes enter view $v$, they send a \textsc{Status} message to all nodes. Thus, all correct nodes will eventually receive $n-f$ \textsc{Status} messages, compute the highest lock, and send a \textsc{Forward-HighestRanked} message to all nodes. Any correct node will echo a \textsc{Forward-HighestRanked} message to all nodes (if it has not done so already). Let $B$ be the set of $f+1$ nodes which have partially synchronous fault-free paths to $L_v$. Since view $v$ is after GST, and every node in $B$ has a partially synchronous fault-free path to $L_v$, every node in $B$ will receive a \textsc{Propose} message from $L_v$ before their echo timer expires. Thus, no node in $B$ will send a \msg{Blame}{v} message. Since a blame certificate requires $n-f$ nodes to send a \textsc{Blame} message, and $f+1$ nodes in $B$ will not send a \msg{Blame}{v} message, no blame certificate will ever form in view $v$. Thus all correct nodes will eventually receive a \textsc{Propose} message, update their local $lock$, and send a \msg{Vote}{v,-} message to all nodes. All correct nodes will eventually receive $n-f$ \msg{Vote}{v,-} messages and terminate in view $v$.
\end{proof}

\begin{theorem}
All correct nodes eventually terminate.    
\end{theorem}

\begin{proof}
If at some point some correct node terminates, it will send a \textsc{Commit} message to all nodes. This message is sent by a correct node, so all correct nodes will eventually receive the \textsc{Commit} message and terminate as well. Now assume that no correct node terminates in any view $v'<v$. In that case by lemma \ref{lem:haps-cft-term-3}, all correct nodes will eventually reach view $v$. Then by lemma \ref{lem:haps-cft-term-4}, all correct nodes terminate during view $v$.
\end{proof}


==> disc_2024/psync-sync-protocols.tex <==





\section{HAPS CFT}

\subsection{HAPS CFT Consensus Utilities}


\par \textbf{Graph Structure.} Our HAPS CFT consensus protocol also uses the $d$ parameter, which is the maximum length of the synchronous fault-free path between any two nodes. 
Our protocol additionally takes advantage of partially synchronous paths from the correct $f+1$-bisource to prevent spurious view changes. We define $d'$ to be the maximum length of the shortest (by length) partially synchronous fault-free path between any two nodes.
We rely on paramter $d'$ so that nodes wait long enough to retrieve data that is in-flight. If $d'$ is known it can be directly used, otherwise, $d'\coloneqq n-f+1$ to account for the worst case when the longest partially synchronous fault-free path consists of all $n-f$ correct nodes.



\par \textbf{Normal Case.} We first focus on the normal case of the protocol, when progress is made. This is guaranteed when the leader of the current view, $v$, is a correct $\diamond f+1$-bisource (after GST). The normal case begins when nodes enter view $v$.

\par \underline{\textit{Begin view step.}}
Upon entering a new view $v$, a node sends a \msg{Status}{v,lock} message to \textbf{all} nodes (Alg. \ref{alg:cft-haps} line \ref{status-haps}). %\natacha{Still to present tense? all nodes broadcasts, eventually, a node receives, etc. Changed it for you already} 
When a node eventually receives at least $n-f$ \msg{Status}{v,-} messages, it calls \textsc{HighestRanked} to find the highest ranked lock from these set of \textsc{Status} messages (Alg. \ref{alg:cft-haps} line \ref{highest-rank-haps}). It then includes this lock in the \textsc{Forward-HighestRanked} message it sends to all nodes (Alg. \ref{alg:cft-haps} line \ref{forward-high-rank}). The node then starts a timer with $2d'\Delta$ duration (Alg. \ref{alg:cft-haps} line \ref{start-echo-timer-haps}). This timer duration ensures that if the leader is a correct $\diamond f+1$-bisource, then all nodes will receive its proposal before its echo timer expires.
%\natacha{Can you make sure to corresponding pseudo code lines? It's a lot to read a full block of text like this}

\par \underline{\textit{Leader proposal step.}} Upon receiving a \msg{Forward-HighestRanked}{v,val} message, the leader checks if $val=\bot$. If $val=\bot$, then no value could have been committed in an earlier view (by quorum intersection any committed value must be the highest ranked value), so the leader can propose its own value, $val_i$. Otherwise if $val\neq \bot$, then the leader must propose $val$ since $val$ could have been committed in an earlier view (Alg. \ref{alg:cft-haps} lines \ref{check-high-rank-haps}-\ref{end-check-high-rank-haps}). The leader sends a \msg{Propose}{v,val} to all nodes (Alg. \ref{alg:cft-haps} line \ref{send-leader-prop-haps}). 

\par \underline{\textit{Receive proposal step.}} In the good case, a node will receive a \msg{Propose}{v,val} message from the leader before its $echo\_timer$ expires. Upon receiving \msg{Propose}{v,val}, the node echoes the \textsc{Propose} message and updates its local $lock=(v,val)$ (Alg. \ref{alg:cft-haps} line \ref{update-lock-haps}). After a node updates its lock, it will \textbf{first} send a \msg{Forward-Propose}{v,val} to all nodes \textit{before} sending a \msg{Vote}{v,val} message to all nodes (Alg. \ref{alg:cft-haps} lines \ref{forward-prop-haps}-\ref{vote-send-haps}). The \textsc{Forward-Propose} message is sent to propagate the leader's proposal to more nodes. 


%\par \textbf{Protocol Description.}
%Our CFT consensus protocol operates in a series of views, where each view consists of a steady state, and a view change procedure to replace leaders suspected to be faulty. The leader of a view can be elected using a simple round robin scheme (node $v \pmod n$ is the leader of view $v$, where $n$ is the total number of nodes). If the leader fails to send its proposal in a timely fashion, nodes will blame the leader and invoke the view change procedure to replace the leader. After each view change, the view is incremented, and the steady state begins again.

%\par \textbf{Utilities.} In our protocol, nodes \textit{lock} on values that could have been committed. A \textit{lock} consists of a view and value, and is used to determine what value a leader must propose. Nodes send their locks using a \textsc{Status} message, which also contains the current view. \textsc{HighestRanked} is a procedure that takes in a set of \textsc{Status} messages from at least $n-f$ nodes, and returns the lock with the highest view. This lock is considered to have the highest rank. We use this to preserve safety as the protocol guarantees that if a value is committed then the highest lock must be for that value. 



%At a first glance it may seem unnecessary to have both \textsc{Forward-Propose} and \textsc{Vote} messages. The problem with just using \textsc{Vote} messages is that a node can crash in the midst of sending \textsc{Vote} messages to all nodes. This can result in one node receiving a quorum of votes and committing, while other nodes may never receive the committed value before moving to the next view. By sending a \textsc{Forward-Propose} message \textit{before} sending a \textsc{Vote} message, we guarantee that even if a node crashes in the process of sending a \textsc{Vote} message to all nodes, it must have sent a message containing the committed value to other nodes. And before moving to the next view, nodes will wait enough time to receive \textsc{Forward-Propose} messages that were in flight. When a node receives a \msg{Forward-Propose}{v,val} message it updates its local lock to the proposal made by the leader \natacha{Is there a possibility of moving this paragraph after you've finished describing the steady state? It's a bit confusing to have half a conversation}.

\par \underline{\textit{Echo proposal step.}} When a node receives a \msg{Forward-Propose}{v,val} message, it updates its local $lock=(v,val)$, and then forwards the \msg{Forward-Propose}{v,val} message to all nodes (Alg. \ref{alg:cft-haps} line \ref{echo-forward-pop-haps}). This echo step is necessary to have the leader's proposal reach at least $f+1$ nodes.

\par \underline{\textit{Commit step.}} When a node receives a quorum of $n-f$ \msg{Vote}{v,val} messages it sends a \msg{Commit}{val} message to all (Alg. \ref{alg:cft-haps} line \ref{send-commit-haps}). Upon receiving a \msg{Commit}{val} message it commits $val$ (Alg. \ref{alg:cft-haps} line \ref{receive-commit-haps}).


\par \textbf{View Change}. 
%\natacha{Is there any chance you could add some structure to the next? Right now it's a wall of text so hard to follow each step?} 
%When the elected leader is not the correct $\diamond f+1$-bisource its proposal may not reach all the nodes. We therefore have a view change protocol that is triggered when at least $n-f$ nodes, suspect the leader is not the correct $\diamond f+1$-bisource or it is before GST and the links of the bisource are not synchronous yet. A quorum of $n-f$ nodes ensures that at least one of the nodes (by quorum intersection) must be one of the $f+1$ nodes that the bisource has partially synchronous links to. This prevents a spurious view change of the correct $\diamond f+1$-bisource after GST.
We have a view change procedure that replaces leaders when they are suspected faulty.


\par \underline{\textit{Trigger Conditions.}} A node suspects the leader is faulty if it does not receive a \msg{Propose}{v,-} message before its echo timer expires. When this occurs, a node then sends a \textsc{Blame} message to all nodes, indicating it wishes to quit the view (Alg. \ref{alg:cft-haps} line \ref{send-blame-haps}). When a node receives $n-f$ \textsc{Blame} messages for the current view, it sends a \textsc{Blame-Cert} message to all nodes (Alg. \ref{alg:cft-haps} line \ref{forward-blame-cert-haps}). Once a node receives a \textsc{Blame-Cert} message, it begins the waiting period.

\par \underline{\textit{Waiting Period.}} When a node receives a \textsc{Blame-Cert} message for the current view, it forwards the message to all nodes, so other nodes will also quit the current view (Alg. \ref{alg:cft-haps} line \ref{forward-blame-cert-haps}). Afterwards, the node waits $2d\Delta$ before moving on to the next view (Alg. \ref{alg:cft-haps} line \ref{wait-period-haps}). During this waiting period, the node will stop accepting \textsc{Propose} messages, and listen for \textsc{Forward-Propose} messages that may have just been sent (Alg. \ref{alg:cft-haps} line \ref{stop-prop-haps}). The waiting period is necessary to ensure that a node will not miss updating its lock before entering the next view.

\par \underline{\textit{Enter next view.}} After the waiting period is over, a node can safely move to the next view (Alg. \ref{alg:cft-haps} line \ref{new-view-haps}). The normal case then resumes.





%When a node receives a \msg{Blame-Cert}{v} message, it forwards this message to all. The \msg{Blame-Cert}{v} message is a ticket for nodes to know they should move on to the next view. However, a node cannot just move to the next view immediately. The reason is that another node may have simultaneously sent a \msg{Vote}{v,val} message. A node that view changes may miss receiving the \msg{Forward-Propose}{v,val} message before entering the next view. This can violate safety, as if $val$ is committed then we need at least $f+1$ nodes to lock on $(v,val)$ before exiting the view. A node thus waits $2d\Delta$ before entering the next view to receive a \textsc{Forward-Propose} message that is in-flight. Upon entering the next view, a node returns to the steady state.

\par \textbf{Analysis.} The correctness proofs are found in Appendix \S\ref{crash-proofs}.

% The reason is that suppose a node in the synchronous connected subgraph receives a \msg{Blame-Cert}{v} message at time $t$. \msg{Blame-Cert}{v} will be received by all nodes in the synchronous connected subgraph by time $t+d\Delta$. This is the latest time a node can send a \msg{Vote}{v,val} message because upon receiving a \msg{Blame-Cert}{v} message a node stops processing \textsc{Propose} messages. We know that the node could at the latest have sent a \msg{Forward-Propose}{v,val} message at time $t+d\Delta$. So since the \msg{Forward-Propose}{v,val} message is multi-casted at time $t+d\Delta$ it is guaranteed to reach all nodes in the synchronous connected subgraph by time $t+2d\Delta$. By waiting $2d\Delta$ before entering the next view, we guarantee that nodes in the synchronous connected subgraph have enough time to process \textsc{Forward-Propose} messages before exiting the view. Upon entering the next view, a node returns to the steady state.

\begin{algorithm}
\begin{algorithmic}[1]
\State{$d\gets $ length of the longest synchronous fault-free path}
\State{$d'\gets $ length of longest partially synchronous fault-free path}
\State{$val_i$}\Comment{The input value of this replica}
\State{$v\gets 1$}\Comment{Current view}
\State{$lock \gets \bot$}\Comment{Highest ranked slow certificate}

\State{$echo\_timer \gets timer(2d'\Delta)$}\Comment{Timer for receiving leader value}

\Event{receiving $S\gets n-f$ \msg{Status}{v,-} messages}
\State{$val \gets \Call{HighestRanked}{S}$}\label{highest-rank-haps}
\State{\textbf{send} \msg{Forward-HighestRanked}{v,val} to all}\label{forward-high-rank}
\State{\textbf{start} $echo\_timer$}\label{start-echo-timer-haps}
\EndEvent

\rl{i am not sure why anyone will have enough status to trigger forward status. Maybe just forward every status to leader?}

\rl{Why set timer in a different place?}

\rl{Can we just say: same as line X to Y?}

\Event{receiving \msg{Forward-HighestRanked}{v,val}}
\State{\textbf{echo} \msg{Forward-HighestRanked}{v,val}}
\If{$i=L_v$}
\If{$val=\bot$}\label{check-high-rank-haps}
\State{$val\gets val_i$}\Comment{If no value could have been committed, propose current input value}
\EndIf\label{end-check-high-rank-haps}
\State{\textbf{send} \msg{Propose}{v,val} to all}\Comment{Leader proposal}\label{send-leader-prop-haps}
\EndIf
\EndEvent

\Event{receiving \msg{Propose}{v,val}}
\State{$lock \gets (v,val)$}\label{update-lock-haps}
\State{\textbf{echo} \msg{Propose}{v,val}}
\State{\textbf{send} \msg{Forward-Propose}{v,val} to all}\label{forward-prop-haps}
\State{\textbf{send} \msg{Vote}{v,val} to all}\label{vote-send-haps}
\EndEvent

\Event{receiving \msg{Forward-Propose}{v',val}}
\State{\textbf{echo} \msg{Forward-Propose}{v',val}}\label{echo-forward-pop-haps}
\If{$v'\geq v$}
\State{$lock \gets (v,val)$}\label{update-forward-prop-haps}
\EndIf
\EndEvent

\Event{receiving $n-f$ \msg{Vote}{v,val}}
\State{\textbf{send} \msg{Commit}{val} to all}\label{send-commit-haps}
\EndEvent

\Event{receiving \msg{Commit}{val}}
\State{\textbf{commit} $val$}\label{receive-commit-haps}
\EndEvent

\Event{$echo\_timer$ expiring and have not received \msg{Propose}{v,-}}
\State{\textbf{send} \msg{Blame}{v} to all}\label{send-blame-haps}
\EndEvent
\rl{Change blame to suspect, and blame-cert to blame? Then I think we can omit some repeated code}

\Event{receiving $n-f$ \msg{Blame}{v'}, where $v'\geq v$}
\State{\textbf{send} \msg{Blame-Cert}{v} to all}\label{send-blame-cert-haps}
\EndEvent

\Event{receiving \msg{Blame-Cert}{v'}, where $v'\geq v$}
\State{\textbf{echo} \msg{Blame-Cert}{v'} to all}\label{forward-blame-cert-haps}
\State{\textbf{wait} $2d\Delta$}\Comment{Wait for Forward-Propose messages to propagate to all replicas in the connected component}\label{wait-period-haps}
\State{\textbf{stop} accepting \textsc{Propose}, do not send \textsc{Vote} messages in view $v'$}\label{stop-prop-haps}
\State{$v\gets v'+1$}\label{new-view-haps}
\State{\textbf{send} \msg{Status}{v,lock} to all}\label{status-haps}
\EndEvent

\end{algorithmic}
\caption{HAPS CFT Consensus Protocol}\label{alg:cft-haps}
\end{algorithm}

==> notes.tex <==
\section{Notes}

\subsection{Problem}
We are given a graph $G=(V,E)$, 
where $V$ contains the set of replicas, and $E$ contains the set of links between 
replicas. We define a subset $F \subset V$ containing replicas which are Byzantine 
faulty. Also, we define a subset $E_1 \subseteq E$ as containing links that are 
synchronous (messages sent on this link arrive within $\Delta$). Similarly, we
define a subset $E_2 \subseteq E$ as containing links that are partially
synchronous (messages sent on this link are only guaranteed to arrive within 
$\Delta$ after GST). $|V|=2|F|+1+A$, where $A \subset V$. 
$|E|=|E_1|+|E_2|$.


\subsection{Conditions for solving consensus.} 
\begin{enumerate}
    %\item Consider the graph $G'=(V \setminus F, E_1)$. If there exists two
    %connected components of size $> A$, then consensus is not possible.
    %\item Consider the graph $G=(V \setminus F, E_1)$. If there exists a
    %connected component of size $\geq |F|+1$, then consensus is possible.
    \item Consider the graph $G=(V \setminus F, E_1)$. If there exists two disconnected
    components of size $> |V|-2|F|$, then consensus is impossible.
\end{enumerate}

\begin{proof}
Consider connected components $P$ and $Q$ of size $|N|-2|F|$ which are disconnected and contain all non-faulty replicas. Nodes in $P$ have input $m$ and nodes in $Q$ have input $M\neq m$. Nodes in $F$ act as having input $m$ to $P$ and act as having input $M$ to $Q$.

World 1: 
\end{proof}

%Conditions 1 and 2 are equivalent.

%\subsection{Protocol Ideas for Known Graph}
%Modify Sync-HS for this setting. The leader uses a flooding type strategy. Each
%replica has a timeout of (diameter)$(2\Delta)$.
%The leader sends a signed message containing its ID to each neighbor. If a vertex
%receives two conflicting proposals from the same ID then it floods the network
%with a \textsc{Blame} message containing the equivocation. If after the timeout
%there is no equivocation, then the neighbor floods the network with \textsc{Vote}
%messages. Each neighbor continually
%signs the message it gets from the leader, including its ID, and forwards it
%to each of its neighbors.

\subsection{Protocol}

\begin{enumerate}
    \item Leader sends \textsc{Propose} message to all replicas containing the highest certificate (fast or slow)
    \item Upon receiving a \textsc{Propose} message
    \begin{enumerate}
        \item A replica sends a \textsc{Fast-Vote} message to all replicas if it is the first proposal it has heard from the leader in the view (after sending a fast-vote a replica does not send another fast-vote in the same view)
        \item A replica sets a timeout for $2\Delta$, and forwards the \textsc{Propose} message to all replicas
    \end{enumerate}
    \item Upon receiving an equivocating proposal or view timer expires (indicating lack of progress in view), cancel timer, send a \textsc{Blame} message containing the equivocating proposals (do not send a \textsc{Vote} or \textsc{Fast-Vote} message)
    \rl{You probably already sent Fast-Vote by now. I usually just say quit view, which means skip all steps below. Is that fine?}
    \item Otherwise, after timer expires and no equivocating proposal was detected or no blame certificate was received, send a \textsc{Vote} message to all replicas
    \item If a replica receives $2f+1$ \textsc{Fast-Vote} messages for the proposal, it forms a fast certificate, and sends the fast certificate to all replicas \rl{is this needed?}
    \item Upon receiving $n-f$ \textsc{Vote} messages form a normal \rl{any reason to consider slow to be the normal path?} certificate, and send the certificate to all replicas
    \item Upon receiving a certificate in the current view (fast or slow), send a \textsc{Fast-Ack} message to all replicas. \rl{This step will be immediately triggered by step 5 oi 6, right?} \rl{Slow cert triggers fast ack? Feels odd.} Start a timer for $1\Delta$. 
    \item Upon receiving $2f+1$ \textsc{Fast-Ack} messages commit the certificate, and send the set of $2f+1$ \textsc{Fast-Ack} messages to all replicas \rl{is this needed?}
    \item After timer expires, send a \textsc{Slow-Ack} message to all replicas
    \item Upon receiving $n-f$ \textsc{Slow-Ack} messages commit the slow certificate, and send the $n-f$ \textsc{Slow-Ack} messages to all replicas
    \item Upon receiving $f+1$ blame messages, form a blame certificate, send blame certificate to all replicas, send a \textsc{Status} message containing the highest certificate by view (fast certificate trumps normal certificate) to the new leader
    \item Leader waits for $n-f$ \textsc{Status} messages and picks the highest certificate by view (normal or fast) to propose
\end{enumerate}

\subsection{Protocol Intuition}
\par \textbf{Why fast quorums of size $(n+f+1)/2?$} Fast quorums don't rely on synchronous equivocation detection, so in order to ensure non-equivocation fast quorums must intersect in at least f+1 replicas (fast quorums intersection is between f+1 and 2f+1 replicas depending on the value of n), of which at least 1 is honest.

\par \textbf{Why slow quorums of size $n-f$?} Since there are $f+1$ honest replicas in the clique there is at most $n-(f+1)=n-f-1$ replicas not in the clique. So a quorum of $n-f$ includes at least one honest replica from the clique. This honest replica in the clique ensures non-equivocation by using the synchronous equivocation detection mechanism.

\par \textbf{Why wait $2\Delta$?} For safety, we need to ensure that there cannot be a fast certificate and a slow certificate for two different proposals in the same view. To satisfy this property we need to guarantee that if a fast certificate forms for a proposal x, then no honest replica in the clique can send a slow vote for a different proposal x'. Otherwise, a slow quorum consisting of 1 honest replica in the clique, f byzantine replicas, and n-2f-1 honest replicas not in the clique could vote for x and a slow certificate for x can form. Since an honest replica in the clique waits $2\Delta$ before sending a slow vote we are guaranteed that it will detect an equivocating proposal for which a fast certificate could have formed. This is the case whether or not this replica is leading or lagging. 

\par \textbf{Why not $1\Delta$?} Suppose a leader sends x to one honest replica in the clique but x' to all other replicas, and a fast certificate for x' forms. All other honest replicas in clique see the proposal for x after they have fast voted for x', and therefore do not slow vote or fast vote. However, the honest replica who voted for x does not see equivocating proposal for x' in time (since it only waits $1\Delta$ and not $2\Delta$) and therefore slow votes for x. Other byzantine replicas and honest replicas not in clique also potentially slow vote x leading to a slow certificate for x.

\par \textbf{Why do we need a second phase?} The problem is that potentially only an honest replica outside of the clique forms a certificate. Therefore if we commit directly once a honest replica forms a certificate is not guaranteed to be received by other honest replicas before a view change occurs (since those links are partially sync). In fully sync protocols we are guaranteed that if an honest replica forms a certificate it will reach all other honest replicas within $\Delta$ after. We don't have that luxury here so we have a second phase to ensure that enough honest replicas have received the certificate before committing.

\par \textbf{Why do you need $2f+1$ fast acks to commit?} A fast ack indicates a replica has received a certificate. In the view change the leader contacts a quorum of $n-f$ replicas. An $n-f$ quorum intersects a $2f+1$ quorum in at least 1 honest replica. This honest replica will send a \textsc{Status} message containing the certificate.

\par \textbf{Why a $1\Delta$ timer before sending a \textsc{Slow-Ack}?} We need to ensure all honest replicas in the clique receive the certificate before sending a \textsc{Slow-Ack}. This is because in the view change the new leader contacts a quorum of $n-f$ replicas, of which at least 1 must be from an honest replica in the clique. So if all the honest replicas in the clique have the certificate before commitment happens on the slow path then this certificate will be seen. $n-f$ \textsc{Slow-Ack} messages indicate that at least 1 is from an honest replica in the clique. This honest replica will propagate the certificate to all other honest replicas in the clique before sending a \textsc{Slow-Ack} message, guaranteeing that the certificate will appear in the view change.

\par \textbf{Why $n-f$ quorum for view change?} The leader can only wait for a maximum of $n-f$ replicas for liveness.


%\par Safety within a view. 1) There cannot exist two fast certificates for conflicting proposals in the same view. A fast certificate requires 2f+1 fast votes. The two fast certificate quorums intersect in at least 1 honest replica. An honest replica never fast votes twice in the same view. 2) There cannot exist two slow certificates for conflicting proposals in the same view. A slow certificate requires n-f votes. At least 1 of these votes must be from an honest replica in the clique. An honest replica sets a timeout for 1Delta before voting, which means that if an honest replica in the clique sent a vote, the other honest replicas in the clique will have detected it and stopped voting. 3) There cannot exist a fast certificate and a slow certificate in the same view. A fast certificate contains 2f+1 votes of which x are from honest replicas in the clique. A slow certificate contains n-f votes of which at least 1 is from an honest replica in the clique. From the 1Delta timeout the leading replica will detect the conflicting proposal and not fast vote or slow vote.

%\par Non-equivocation lemmas - Lemma 1: There cannot exist two fast certificates for conflicting proposals in the same view. Proof: A fast certificate requires 2f+1 fast votes. The two fast certificate quorums intersect in at least 1 honest replica. An honest replica never fast votes twice in the same view. Lemma 2: There cannot exist two slow certificates for conflicting proposals in the same view.
%There cannot exist a fast certificate and a slow certificate for conflicting proposals in the same view. 

%Case 1) Honest replica in clique fast votes for x first, sets timeout for 1Delta, other honest replica in clique sees the proposal for x and therefore does not vote for x'
%Case 2) Honest replica in clique slow votes for x' first, sets timeout for 1Delta, but within the timeout the other honest replica in the clique fast votes for x before equivocation is detected



%\subsection{Protocol for Unknown Graph}
\subsection{Good Case Latency Lower Bound}
Good case: After GST with an honest broadcaster.
Theorem: It's impossible to solve consensus in less than 3 rounds in almost partial synchrony
Proof: Suppose there exists a protocol that solves consensus in 2 rounds. Let P be replicas in the synchronous connected component, Q be the other honest replicas, and F the faulty replicas. World 1: Before GST, P and Q are partitioned and they receive the same value. They both have to commit after receiving n-f responses after 2 rounds. Messages from Q to P are delayed indefinitely but messages from P to Q are received in time. This causes Q to commit.

Suppose 1<=|P|<=f, |F|=f, and |Q| = f

World 1: Q, F are honest. P is byzantine. After GST broadcaster is honest with input x. 
Parties in P act crashed.
Broadcaster sends value to all parties in round 1. In round 2 all parties do an all to all exchange. At the end of of round 2, parties in Q must decide by the good case latency property. Q receives messages that said they heard x from Q, and F. By the good case latency property Q must decide x.

World Hybrid: P, Q are honest. F is byzantine. Before GST broadcaster is dishonest. Suppose messages from Q to P are delayed (before GST). Q receives messages from Q, and F containing x. From Q's perspective World 1 and World Hybrid are indistinguishable, so since Q commits x in World 1, Q must commit x in World Hybrid. P receives messages from F indicating the broadcaster equivocated. 

\begin{itemize}
    \item Any set of n-f must have fault free sync paths to a set of at least $f+1$ nodes
    \item Suppose not, then there exists at least 1 set of n-f with fault free sync paths to at most $f$ nodes. Let this set of $f$ nodes be $S$, and the remaining $n-f\leq f$ nodes be $T$.
    \item Any path from $S$ to $T$ is either 1) synchronous with faulty nodes in the path or 2) async
    \item If a path consists of faulty nodes cannot distinguish between sync and crashed vs async and correct path
    \item Have one world which is async and correct (hybrid) and another world which has sync and crashed
    \item Have two sets, S and T with cardinality <= f but which are only sync connected by faulty nodes
    \item Suppose S - F - T. Essentially make F a part of set T. S non-faulty world 1. In world hybrid F crashes. The problem is if F crashes at the beginning then messages between F and T are no longer sync
    \item suppose n=5, f=3, n-f=2 Have an A - B - C connected component, B is faulty, D, E in their own connected components, n-f quorum A, D, reaches nodes A, B, D = 3 nodes <= f = partition set S. partition set T consists of C and E <= f
    \item in this case there is a set of n-f that reaches n-f+1 nodes but n-f+1<=f, f-1 other nodes
    \item we know any set of n-f must reach at least n-f nodes. any additional nodes it reaches must subtract from the total number of faulty nodes
    \item let c be the number of additional correct nodes n-f is connected to, and k be the number of additional faulty nodes n-f is connected to
    \item consider the remaining f-c-k nodes in the other partition
    \item Set S is n-f+c nodes. Set T is f-c-k nodes. Set R is set k of faulty nodes. All three sets are disjoint and add up to n nodes
    \item World 1: S is honest, T and R are crashed = f-c nodes are crashed.
    \item World 2: T is honest, S and R are crashed = n-f+c+k <= f nodes by assumption
    \item World Hybrid: S and T are honest, R is crashed = k nodes <= f. Split brain succeeds
    \item Let S be set of nodes that n-f is sync connected to by fault-free paths (must be at least n-f since nodes trivially have sync edge to themselves). Let S' be the set of nodes n-f is sync connected to (including paths with faulty nodes). 
    \item Let k be the number of faulty nodes in S s.t. if k was non-faulty, S would = S'
    \item Define sets S, k, and remaining T nodes
    \item nodes in k are always crashed across all worlds, split brain S and T
    \item Consider set of n-f nodes. These n-f nodes must have a sync fault-free paths to themselves (n-f). Consider the other nodes in $S$ not apart of the n-f set which are faulty
    \item Consider set of $\leq f$ nodes which $n-f$ are fault free sync connected to ($S$). There is a max of $n-f$ in the other partition ($T$). Note that $n\leq 2f$, so $n-f\leq f$
    \item Let $R$ be set of faulty nodes in $S$ not in the original $n-f$ which are sync connected to nodes in $T$
    \item Need to show that $|T|+|R|\leq f$, we know $T=|n-f$ but how to bound $R$, if we assume $|R|=2f-n$, then $|T|+|R|=n-f+2f-n = f$, which works out
    \item Any sync non-fault-free path from S to T must involve one of the nodes in R
    
\end{itemize}

\begin{itemize}
    \item Any set of n-f must have fault free sync paths to a set of at least $f+1$ nodes
    \item Suppose not, then there exists at least 1 set of n-f with fault free sync paths to at most $f$ nodes. Let this set of $f$ nodes be $S$, and the original set be $O$ and the remaining $n-f\leq f$ nodes be $T$.
    \item Let $R$ be a subset of $S$ containing the faulty nodes node in $S$
    \item World 1. Let S - R be non-faulty. Let R and T be crashed. Since $O$ is at least n-f, then R U T is at most f.
    \item World 2. Let T be non-faulty. Let S be crashed. S by definition is <= f.
\end{itemize}

Notes:
Condition: Graph G must have at least 1 $f+1$ psync bisource and any set of n-f must have sync fault-free paths to at least f+1 nodes

Proof: Suppose for contradiction that G has at most $f$ psync bisources or there does exist a a set of n-f that is sync connected to at most f nodes.
Case 1: There does exist a set of n-f which is sync connected to at most f nodes. Then execute split brain attack before GST
Case 2: There are only $f$ psync bisources but any set of $n-f$ is sync connected to at least $f+1$.
Suppose for contradiction there exists an algorithm that solves consensus for this graph. Construct another graph G' which has $f+1$ nodes of which $1$ is faulty. We augment G' to have $f$ more nodes but 
f+1-(n-f) = 2f+1-n, but 

We want to start with graph that x nodes with 1 faulty which is fully async, and add some fake nodes to have a graph that has n-f sync connected to f+1, and also have f psync bisources. 
The old graph has a set C of n-f-1 correct nodes with no sync/psync links, and a set F of 1 faulty node. Then we add a set S of f-1 fake nodes that are crashed. We split S into two disjoint subsets: S1 and S2. S1 contains 2f+1-n nodes. And S2 has the remaining nodes. Each node in C has sync links to every node in S1. 

We need to guarantee ANY set of n-f has sync fault-free paths to at least f+1 nodes

we add 2f+1-n fake nodes. Each of the old nodes in the graph have a sync link to the fake nodes. Any set of n-f nodes should have sync fault-free paths to f+1 nodes. 
Then add another set of f-1-(2f+1-n)= f-1-2f-1+n = n-f-2 fake nodes

Counterexample:
Suppose n=6, f=3, any set of 3 nodes needs to be connected to 4 nodes
R1 R2 R3
|  |  |
R4 R5 R6
In this graph no f+1 bisource (every node sync connected to f-1=2 nodes)
How can we reduce this to FLP?
We are allowed to add any set of f-1 (2) fake nodes to the original graph

R1, R2 are correct, R3 is faulty (n=2f+1, f=1)
Add fictious nodes

Suppose n=6, f=3, any set of 3 nodes must have sync fault free paths to 4 nodes
R1 R2 R3 R4
| |  | | |
R5  R6

R1 sync edges to R5, R6
R2 sync edges to R5, R6
R3 sync edges to R5, R6
R4 sync edges to R5, R6

Reduce to FLP, where R1, R2, R3 are correct, R4 is crashed, R5, R6 are fictious. Note that there are no sync edges between R1, R2, R3, R4, R5, R6

Note that it doesn't work for n=f+1 because in that case we need a connected component which is equivalent to a bisource

f+1 - (n-f-1) = f+1-n+f+1 = 2f+1-n

f+1 psync bisource
it breaks down because to make everyone an f+1 bisource you need at least f dummy nodes (each node has psync trivially to itself, and then f other nodes) but you can't have more than f faulty nodes

n-f-2, 1

suppose for contradiction no f+1 psync bisource but any set of n-2f honest has sync fault free paths to f+1 honest
n=10, f=4, n=2.5f
6 honest
construct graph where any set of 2 honest is sync connected to 5 honest but no one honest is sync connected to 5 honest

R1 - R2 - R3
      |
R4 - R5 - R6

If n-2f=f, where f=5, then n=15, 10 correct, any set of 5 (n-2f=15-10=5) correct must be connected to 6 (f+1=5+1=6) but no single correct node can be connected to 6
Example graph as to why you need an f+1 psync bisource
R1 - R2

R3 - R4 - R5 - R6

R7 - R8 - R9 - R10

Divide correct nodes into groups of f-1, if n-2f=f then the first n-2f-1 is connected to f-1, and the last of the nodes is connected to additional f-1, since 2(f-1)>=f+1 then n-2f is connected to at least f+1 correct

This graph also works
R1 - R2
R3 - R4
R5 - R6
R7 - R8
R9 - R10

Consensus => (A AND B)
not Consensus OR (A AND B)

Contradiction
not (not Consensus OR (A AND B)) =
Consensus AND not(A AND B) = 
Consensus AND (not A OR not B)

